Near Optimal Dual Fault Tolerant Distance Oracle

We present a dual fault-tolerant distance oracle for undirected and unweighted graphs. Given a set $F$ of two edges, as well as a source node $s$ and a destination node $t$, our oracle returns the length of the shortest path from $s$ to $t$ that avoids $F$ in $O(1)$ time with a high probability. The space complexity of our oracle is $\Tilde{O}(n^2)$ \footnote{$\Tilde{O}$ hides poly$\log n$ factor }, making it nearly optimal in terms of both space and query time. Prior to our work, Pettie and Duan [SODA 2009] designed a dual fault-tolerant distance oracle that required $\Tilde{O}(n^2)$ space and $O(\log n)$ query time. In addition to improving the query time, our oracle is much simpler than the previous approach.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> OneFault.tex <==
\section{Oracle for single fault}
In this section, we discuss the oracle to find the distance between two vertices $s,t$ avoiding an edge $e$. Initially, we design an oracle with size \OO$(n^4)$. After that, we will modify it to size \OO$(n^2)$. The query time for both of the oracle is $O(1)$.
We will store the following data-structures during the preprocessing phase.
\begin{enumerate}
	\item The breadth first search tree, $\BFS(u)$, from all $u \in V$.  This takes $O(n^2)$ space. 
	
	\item The $\FT(uv)$ data-structure of \cite{Chechik18} for all pair of vertices in $G$. Since the size of each $\FT(\cdot)$ structure is $\TL(1)$, the total size of all the $\FT$ data-structures is  $\tilde{O}(n^2)$.

	\item $\DD(st,d)$ is a tuple for all pair of vertices in $G$ such that   $d \in [1,n]$. If $e^* = \DD(st,d)$, then we also store the path $st \DIA e^*$ in $\DD(st,d)$. Using \ref{}, $st \DIA e^*$ is a concatenation of atmost 2 shortest paths. Since we have already calculated the shortest path between every pair of vertices, the space required for $\DD(st,d)$, that is the edge $e^*$ as well as the path $st \DIA e^*$  requires $O(1)$ space. 
	As there are $n^3$ possible maximiser tuples, the size of this  data structure is $\tilde{O}(n^3)$. 
	
\end{enumerate}



\subsection{Query Algorithm} 

We now describe the query algorithm. Given a $s$, $t$ and $e$, our algorithm will return $|st \DIA e|$. For brevity we will use the following setting in the lemmas that will follow in this section. This will make the statement of our lemma short.\\  
\textbf{Settings used in the lemmas: }
Let us assume that $P=st \diamond e$ and $e = (u,v)$. 
 Assume wlog that $d = |su| \le |sv| $. We use the maximizer data structure and get $e^* = \DD(st,d)$. Let  $e^*=(p,q)$. Let us assume wlog that $d =|sp| \le |sq|$. There are two cases, depending on whether $e^*$ lies on $P$ or not.  
 \begin{lemma}
 \label{lem:inpath}
 	If $e^* \notin P$, then $ |st \DIA e^*| = |P|$.
 \end{lemma}
 \begin{proof}
Since $P$ avoids $e^*$, $|st \DIA e^*| \le |P|$. Since edge $e$ also satisfies the conditions of the maximizer $\DD(st,d)$, $|P| = |st \DIA e| \le |st \DIA e^*|$. The last two inequalities implies that $|st \DIA e^*|=|P|$.
 \end{proof}
 
Using \Cref{lem:inpath}, if 
 $e^* \notin P$, then we can  return $|st \DIA e^*|$ stored in $\DD(st,d)$. Let us now look at the case when  $e^* \in P$.  We now prove the following lemmas:
 

	

\begin{lemma}
\label{lem:notinsp}
Let $e^* \in P$. Then $e$ cannot lie on both $sp$ and $P[sp]=sp$. 
\end{lemma}
\begin{proof}
Since $|sp| \le |sq|$, $p$ appears before $q$ on $P$.
	 If the shortest path $sp$ passes through $e$, then since $|su| = d$, $|sp| > d$. But we know that $|sp| =d$. So, $sp$ does not pass through $e$. But the path $P[s,p]$ also does not pass through $e$. Thus, $P[s,p]=sp$. 

\end{proof}


\begin{lemma}
\label{lem:trapezoid}
If $e^* \in P$ then, $u,v \notin  \TR_{G-e}(P[p,t])~ $. 
\end{lemma}

\begin{figure}[hpt!]

\centering
\begin{tikzpicture}[]
\coordinate (s) at (0,0);
\coordinate (t) at (8,0);
\coordinate (u) at (3,1);
\coordinate (v) at (4,1.5);
\coordinate (p) at (4,0);
\coordinate (x) at (2.5,0);
\draw (p) node [below] {$p$};
\draw (x) node [below] {$x$};

\draw (s) node[left] () {$s$} -- (t) node[right] () {$t$};
\draw (u) [red] node[left][black] () {$u$} -- (v) node[right][black] () {$v$};
\filldraw [red][opacity=0.15] (x) circle (1.3);
\filldraw [blue][] (p) circle (2 pt);
\filldraw [blue][] (x) circle (2 pt);
\filldraw [blue][] (t) circle (2 pt);
\filldraw [blue][] (s) circle (2 pt);
%\draw[densely dashed] (t) -- (u) ;
\draw[densely dashed] (x) -- (u) ;
%\draw (6,0) node[below] {$d_2$};
%\draw (6,0.5) node[above] {$\leq d_2+1$};
%\filldraw [red] (s) circle (2pt);
%\filldraw [red] (t) circle (2pt);
%\draw  (u) arc(90:-90:1) [ thick,blue];
%\draw  (u) arc(90:-90:1) [ line width=2mm,blue,opacity=0.5];
%\draw (e) node[left] () {$e$} pic[rotate = 0] {cross=3pt};
%\draw (u) node [left] {$u$};
%\draw (v) node[left] {$v$};
\end{tikzpicture}
\caption{Replacement path $(u,v) \diamond e$.}
\end{figure}


\begin{proof}
\begin{comment}
	 For contradiction, let us assume that $u \in \TR(P[s,p] )$. Then, there is a vertex $x \in P[s,p]$ such that $|xu| \le \epsilon\min \{|P[s,x]|, |P[x,p]| \}$.  Consider the following path from $s$ to $u$:	\begin{align*}
		|P[s,x]|  + |xu| &\le  |P[s,x]| +\epsilon \min\{|P[s,x]|,|P[x,p]|\}\\
		& \le |P[s,x]| +\epsilon |P[x,p]|
		\intertext{Assuming  $\epsilon \leq \frac{1}{4}$, if $|P[x,p]| \le 4$, then the ball centering $x$ can not contain any vertex inside. So, let us assume that  $|P[x,p]| > 4$. This imples that $\EP |P[x,p]| \le |P[x,p]|-3$}
		& \le  |P[s,x]| + |P[x,p]|-3\\
		& \le |P[x,p]| - 3\\
		& \le |sp| -3\\
		& = d-3
	\end{align*}
	This implies that there is a path from $s$ to $u$ of length $\le d_1-3$. But this leads to a contradiction because $ |su| = d$. 

\end{comment}
 For contradiction, assume that $u \in \TR_{G-e}(P[p,t])$. This implies that there exists a vertex $x \in P[p,t]$ such that $|xu| \le \min\{|px|,|xt|\}$ and $xu$ does not pass through $e$. We will now show an alternate path from $s$ to $t$ avoiding $e$ whose length is less than $|P|$. Consider that path $su \DIA e + ux + P[x,t]$. The reader can check that all the three components of this path avoid $e$. 
	
\begin{align*}
	|su \DIA e| + |ux| + |P[x,t]| & \le d + \EP\min\{||P[p,x]|,|P[x,t]|\} + |P[x,t]|\\
	&\le d + \EP |P[p,x]| + P[x,t]\\
	&\le |P[s,p]| + \EP |P[p,x]| + |P[x,t]|\\
	& < |P[s,p]| + |P[p,x]| + |P[x,t]|\\
	&=P[s,t]
\end{align*}

We will now show that $v \notin \TR_{G-e}(P)$. For contradiction, assume that $v$ is in the trapezoid.  This implies that there exists a vertex $x \in P[p,t]$ such that $|xv| \le \min\{|px|,|xt|\}$ and $xv$ does not pass through $e$. We will now show an alternate path from $s$ to $t$ avoiding $e^*$ whose length is less than $|P| \le |st \DIA e^*|$. Consider that path $sv + vx + P[x,t]$. The second and the third path donot pass through $e^*$. We will now show that even the first path does not pass through $e^*$. Assume that the first path passes through $e^*$, then its length is $> d+1$. But the length of $|sv| \le |su|+1 = d+1$. Thus, $sv$ does not pass through $e^*$.

\begin{align*}
	|sv| + |vx| + |P[x,t]| & \le d+1 + \EP\min\{||P[p,x]|,|P[x,t]|\} + |P[x,t]|\\
	&\le d + \EP |P[p,x]| + P[x,t]\\
	&\le |P[s,p]| + \EP |P[p,x]| + |P[x,t]|\\
				\intertext{Assuming  $\epsilon \leq \frac{1}{4}$, if $|P[x,p]| \le 4$, then the ball centering $x$ can not contain any vertex inside. So, let us assume that  $|P[x,p]| > 4$. This imples that $\EP |P[x,p]| \le |P[x,p]|-3$}\\
	& < |P[s,p]| + |P[p,x]|-3 + |P[x,t]|\\
	&=P[s,t]
\end{align*}
Since $|st \DIA e^*| \ge |P|$, we arrive at a contradiction.
\end{proof}

Using the above lemma, if $e^* \in P$, then $u$ and $v$ do not lie in $\TR_{G-e}(P[p,t])$. Using \Cref{lem:notinsp}, $P[s,p] = sp$. We combine these two fact to find in the following algorithm. 

\begin{algorithm}[H]\caption{$\QU(s,t,e)$: Returns the distance between $s$ and $t$ avoiding the edge $e$ }
	$d = \min\{|su|,|sv|\}$\;
	$e^*=  \DD(st,d)$ \;
	\tcc{If $e^*$ is not on the path $P$}
	$\AN= |st \DIA e^*|$\; 
	\tcc{If $e^*$ is on the path $P$}
	\If{$e^* \neq e$}
	{
		Let $e^*=(p,q)$\;
		Let us assume wlog that $|sp| \le |sq|$ and $|su| \le |sv|$\;
		$\AN =  \min\{\AN, |sp| + \QFT(pt,e)\}$\;

	}
	\textbf{return} $\AN$ \;
\end{algorithm}

\subsection{Running time of query algorithm} 

We query the $\FT$ data-structure twice in our algorithm. Apart from that, we access our mazimizer data-structure that takes $O(1)$ time. Using \Cref{lem:qft}, the time taken by $\QFT()$ is $O(1)$. Hence, the query time of our algorithm is $O(1)$.


\section{Reducing the space to $\TL(n^2)$}
In the previous section, except for the maximizer data-structure, all other data-structures were of size \OO$(n^2)$. Apart from the maximizer data-structure, we will reuse all the data-structures in the previous section. In this section, we will see how to modify the maximizer data-structure.
We will use the following additional data-structures:


\begin{enumerate}
	\item Landmark vertices $\LL_i$ sampled from $G$ with probability $O\left(\frac{1}{2^i}\right)$ for $i=0$ to $\log n$. The size of each $\LL_i$ will be $\TL\left(\frac{n}{2^i}\right)$. 
	\item For each shortest path, we will store the vertex nearest to $s$ and $t$ that lies in $\LL_i$, where $0 \le i \le \log n$. This requires $O(\log n)$ space per pair. Thus, the total space required is $\TL(n^2)$.
	\item To simplify notations that will follow, we will use $s^i$ as a shorthand to  denote  $s \in \LL_i$.
	

	\item $\DD(s^it^j,d)$ is a tuple for all pair of vertices in $G$ with the following properties: 
	\begin{enumerate}
	\item If $i=0$, then $d_1 = 2^k$ for $0 \le k \le \log n$. Unlike the previous section, where $d_1$ can take $n$ values. Here $d_1$ can take only $\log n$  values. Similarly, when $j=0$, then $d_2 = 2^k$ where $0 \le k \le \log n$.
	\item If $i>0$, then $d_1 \le 2^{i+2}$. Similarly, if $j >0$, then $d_2 \le 2^{j+2}$.
	\end{enumerate}
	
	We define the maximizer as follows:

	\[\DD(s^it^j, d_1,d_2) = \text{argmax}_{e \in E} \begin{cases}|st \DIA e| ~ \text{such that}\\
	d_1 \le |se| \le 2d_1 \hspace{1cm} \text{if $i=0$}\\
	|se| \le d_1 \hspace{1.95cm} \text{if $i>0$}\\
 	d_2 \le |te| \le 2d_2 \hspace{1cm} \text{if $j=0$}\\
	|se| \le d_2 \hspace{1.95cm} \text{if $j>0$}\\
 	\end{cases}
\]
		
\end{enumerate}

If $i=0$, then $d_1$ can take $\log n$ different values. Else, it can take $O(2^i)$ different values. In general, for any $i$, $d_1$ can take $\TL(2^i)$ different values. Similarly, for any $j$, $d_2$ can take $\TL(2^j)$ different values. Since the size of $\LL_i$ and $\LL_j$ is $\TL(\frac{n}{2^i})$ and $\TL(\frac{n}{2^j})$ respectively, for a fixed $i$ and $j$, the size of the maximizer data-structure is $\TL(n^2)$. As there are $\log^2 n$ different $i,j$ pair, the total size of our maximizer data-structure is $\TL(n^2)$.


\subsection{Query Algorithm} 

Given a $s$, $t$ and $e$, our query algorithm will return $P= |st \DIA e|$. In the previous section, in the query algorithm, we used the maximiser $\DD(st,|se|,|te|)$. Uunfortunately, such a maximiser may not exists now. Our aim will be to find nodes, say $r_1^k$ and $r_2^\EL$ on the path $P$ such that (1) $|s r_1|$ and $|r_2t|$ does not contain $e$, (2) $|r_1e| \le 2^{k+2}$ and (3) $|r_2e| \le 2^{\EL+2}$. In that case, we can use maximiser $\DD(r_1r_2, |r_1e|, |r_2e|)$ and run our algorihm in the previous section to find the length $|r_1r_2 \DIA e|$ path. Adding $|sr_1|$ and $|r_2t|$ will give us $|st \DIA e|$. 

 Our query algorithm starts when we call $\QU(s^0t^0,e)$. We set $d_1 = 2^{\lfloor \log |se|\rfloor}$ and $d_2 = 2^{\lfloor \log |te| \rfloor}$. Now, we use our maximiser data-structure and find  $e^* = \DD(s^0t^0,d_1,d_2)$. Let $e^*=(p,q)$. If $e^* \notin P$, then using \Cref{lem:inpath}, we can return $st \DIA e^*$. If $e \in P$, then using \Cref{lem:eitherinsporpt}, there are following two cases:

\begin{enumerate}

\item $sp$ does not contain $e$ 


%\begin{enumerate}
%\item $|sp| \ge |se|$

%Using \Cref{lem:trapezoid},  $\TR(P[p,t])$ does not contain any endpoints of $e$. \todo{Why? We have not proved this in \Cref{lem:trapezoid}. May be we need to rewrite it.} So, the length of $P[p,t]$ can be found by querying the $\QFT(pt,e)$. To this end, we return $|sp| +\QU(p^0t^0, \phi,X \cup F)$. The reader can check that the function $\QU(p^0t^0,\phi,X\cup F)$ basically returns $\QFT(pt,e)$. 

%\item $|sp| < |se|$ but $|sp| \ge d_1$

 Let $d_1 = 2^k$. On the $sp$ path, we find the vertex $r_1 \in \LL_k$ nearest to $p$ . Note that such a vertex exists with a high probability as $|sp| \ge d_1$. Also,  with high probability, $|r_1p| \leq 2^k$. Now, we divide the path $P$ in parts $P[s,r_1]$ and $P[r_1,t]$. We find find the length of these two paths seperately. For $P[s,r_1]$, we can just return $|sr_1|$. For  $P[r,t]$, we recursively call the data structure $\QU(r^kt^0,e)$. \


 %where $d_3= \min \{ d(l_i,a),d(l_i,b) \}$ and $2^j$ is such that, $2^j \leq \min \{ d(v,a), d(v,b) \} \leq 2^{j+1}$. By definition, we either get the maximising edge $e_2$ on the path $P[l_i,v]$ or we get the path itself as the maximum element. Now, if $e_2=(p,q)$ is on that path and the path from $l_i$ to $p$ has no fault then we are ready with the asnwer by following previous arguments. This is because $P[l_i,v]=d(l_i,p)+FT(p,v)(e)$ in that case. 
\item $pt$ does not contain $e$

Similar to the above case.

\end{enumerate}






From the above discussion, the reader can see that either we get the correct answer (if $e^* \notin P$) or case (1): we find  $r_1$ and recurse into either $\QU(r_1^kt^0,e)$ or case (2): we find $r_2$ and recurse into $\QU(s^0r_2^k,F,X)$. Let us assume that we recurse into $\QU(r_1^kt^0,e)$. We first show that   $|r_1^ke| \le 2^{k+2}$. This

\begin{lemma}
$|r_1^ke| \le 2^{k+2}$. 
\end{lemma}
\todo{Dipan, please write this lemma properly as well as the proof.}

\begin{proof}
	
\end{proof}

Let us now look at what happens when we call $\QU(r_1^kt^0,e)$. First note that $d_1 = |r_1e|$ and $d_2 = 2^{\lfloor \log |te| \rfloor}$. And, we have a maximser in our data-structure $\DD(r_1^kt^0,d_1,d_2)$. Let $e^* = (p,q) = \DD(r_1^kt^0,d_1,d_2)$.  If $e^* \notin P[r_1,t]$, then using \Cref{lem:inpath}, we can find the length of the path $P[r_1,t]$. Else, using \Cref{lem:eitherinsporpt}, we claim that either $r_1p$ or $pt$ do not contain $e$. Let go through both the cases:
\begin{enumerate}
	\item $r_1p$ does not contain $e$.
	
	In this case, using \Cref{lem:trapezoid}, we can show that the $\TR(P[p,t])$ does not contain $e$. Thus, we  call $\QFT(r_1t,e)$ and returns the correct $|r_1t \DIA e|$ path.
	
	\item $pt$ does not contain $e$.
	
	In this case, we find a $r_2^{\EL}$ (for some $\EL$) with the guarantee that $|r_2e| \le 2^{\EL+2}$ (similar to \Cref{}). We then recurse into $\QU(r_1^kr_2^\EL, e)$. 
\end{enumerate}

The reader can check that $\QU(r_1^kr_2^\EL,e)$ is our base case, where we do not recurse and return an answer.
























==> algorithm.tex <==
\input{fig_departing}

Let us see how we find and store lengths of the replacement paths at the root of $\TT$, that contains graph $\GG$. First, we find the replacement paths for edges on the primary path. Let $R = st \DIA e$ where $e \in \PP$.  We define $R$ to be either {\em jumping} or {\em departing} depending on whether it merges back to the primary path or not.

\begin{definition}(Jumping and Departing paths)
   Let $R = st \DIA e$ where $e \in \PP$ . $R$ is called a \textbf{\em jumping path} if it uses some vertex $u \in \PP$  after $e$. If the path is not jumping then it is a \textbf{\em departing path}. If a replacement path is jumping, then it is called {\em jumping replacement path}. Similarly, we define departing replacement path. See \Cref{fig:departingjumping}
for a visualization of these two kinds of paths.\end{definition}



Note that, jumping or departing path is defined only when the edge fault is on the primary path. Also,  if a replacement path is departing, then the destination $t$ cannot lie on $\PP$. In \Cref{sec:detail}, we will find all jumping replacement paths.

In  \Cref{sec:departing}, we design a new algorithm for finding and storing all departing replacement paths. To this end, we will use the main idea in the paper of Gupta and Singh \cite{GuptaS18}.  In \cite{GuptaS18}, the authors  sampled a set of  vertices  with probability of $\OO(\frac{1}{\sqrt{n}})$. Then, for a vertex $t \in \GG$, they find a sampled vertex near  $t$ on the $st$ path. They call this vertex  $t_s$. Then, they  show the following important lemma, which is the main idea of their paper:

\begin{lemma} (Lemma 11 in \cite{GuptaS18})
\label{lem:guptaaditi}
The number of replacement paths  from $s$ to $t$ that avoid edges in $st_s$ path and also avoid $t_s$  is $O(\sqrt n)$.
\end{lemma}

An astute reader can see that the definition of replacement paths in the above definition looks very similar to departing replacement paths. We prove that this is indeed the case. Thus, we can transfer the result in \Cref{lem:guptaaditi} to departing replacement paths. This is the main novelty of the paper. The main technical result of \Cref{sec:departing} is as follows:

\begin{lemma}
\label{lem:departing}
For each  $t \in \GG$, all departing replacement paths to $t$ can be found in deterministic $\TL(m\sqrt n)$ time. Moreover, the length of all such departing paths can be stored in a data structure of size $\TL(n\sqrt n)$ and can be queried in $\TL(1)$ time.
\end{lemma}

\input{fig_gmgn}
\section{Algorithm to build SDO(1): Replacement paths that are not departing}
\label{sec:detail}
In \Cref{sec:departing}, we will find all and store all departing replacement paths.
Thus, we just need to concentrate on the replacement paths that are either jumping or the faulty edge $e \notin \PP$.
We now divide remaining replacement paths depending on where the destination $t$ and faulty edge $e$ lies. There are  following cases:


\subsection{$e \in \GM$ and $t \in \GN$}
\label{sec:gmgn}


This case itself can be divided into two cases depending on whether $e$ lies on the primary path or not.
\begin{enumerate}
    \item $e \in \PP$ (See  \Cref{fig:gmgn}(a))


Let $R = st \DIA e$.
If $R$ is departing then we will see how to find it in  \Cref{sec:departing}. So, assume that $R$ is jumping . This implies that $R$ merges back to $\PP$ at a vertex, say $w$, after the edge $e$. Since $t \in \GN$, $st = sw + wr + rt$.  Thus, after merging with $\PP$ at $w$, the replacement path passes through $r$. In that case, $|st \DIA e| = |sr \DIA e| + |rt|$. We can easily find the right hand side of the above equality as we have stored $d(s,r,e) = |sr \DIA e|$ and $d(r,t) = |rt|$.

\item $e \notin \PP$ (See  \Cref{fig:gmgn}(b))



In this case, we claim that $st \DIA e = st$. The $st$ path has $\PP$ as its prefix. Since $\PP$ lies in $\GM$ and survives after the deletion of $e$, $st$ path remains intact.


\end{enumerate}


\subsection{$e \in \GM$ and $t \in \GM$}
\label{subsec:MM}
\input{fig_gmgmcase1}

Since both $e$ and $t$ lie in $\GM$, one may think that we can recurse our algorithm in $\GM$ to find $st \DIA e$.
If $st \DIA e$ completely lies inside $\GM$, this is indeed the case. However,  $st \DIA e$ may also use edges of $\GN$.
To handle such cases, before recursing in $\GM$, we will add weighted edges to it. For each $v \in \GM$, we will add an edge from $r$ to $v$ with a weight $|rv \DIA \GM|$.
We have already calculated this weight, it is stored in $d(r,v,\GM)$.  Let the set of weighted edges added to $\GM$  be called $X$. 
We now look at two cases, (1) $e \in \PP$ and (2) $e \notin \PP$.

\subsubsection{$e \in \PP$ }
\label{sec:gmgmp}
Let $R = st \DIA e$ be a jumping replacement path.
 We will show that $st \DIA e = sr \DIA e + rt$. As we have calculated the length of both the paths in the right-hand side of the above equality, there is no need to even recurse in this case. To prove the above equality, we first prove the following simple lemma:

\begin{lemma}
\label{lem:passr}
Let $e \in  \PP$,  $t \in \GM$. Assume that   the jumping replacement path $R =st \DIA e$ uses some edges of $\GN$. Then $st \DIA e$ passes through $r$.
\end{lemma}

\begin{proof}
Since $R$ is jumping, it merges with $\PP$.  There are two ways in which $R$ can merge with $\PP$.
\begin{enumerate}
    \item $R$ merges with $\PP$ and then visits the edges of $\GN$.



    Let us assume that $u$ is the last vertex of $\GN$ in the path  $R$ and $R$  merges with $\PP$ at $w$. Since $R$ first merges with  $\PP$ and then  visits the  edges of $\GN$, $u$ comes after $w$ on $R$. Since $w$ is below $e$ on $\PP$, we claim that the sub-path $wu$ of $su$ survives in $\GG\setminus e$ and is also the shortest path from $w$ to $u$. But  $wu$ path passes through $r$. Thus, $st \DIA e$ passes through $r$ by construction in \Cref{lem:separator}.

 %Let $v$ be the vertex just after $u$ in $R$. So, $v \in \GM$ and by construction $R[v,t]$ completely lies in $\GM$. Thus, we can write $R$ as $R = R[s,w] + R[w,u] + (u,v) + R[v,t]$. Thus, we can see that $R$ visits $\GN$ just once.

 %Also, $R[w,u] = wu$ and can be written as: $R[w,u] = R[w,r]+R[r,u]$. Thus,
 %\begin{tabbing}
 %$R$\=$= R[s,w] + R[w,r] + R[r,u] + (u,v) %+ R[v,t]$\\
 %\>$ = R[s,r] + R[r,v] +R[v,t]$
 %\end{tabbing}

 %By construction, the first and the last summand of the above equality completely lie in $\GM$ and the middle summand $R[s,v]$
 %does not have any edge of $\GM$. Thus, $R[s,v] = |sv \DIA \GM| = d(r,v,\GM)$. Since, we have added an edge from $r \to v$ with weight  $d(r,v, \GM)$, we claim that there is a path in $\GM \cup X$ that avoids $e$ and has length $R$.

  %The first and the last summand of the previous equality completely lies in $\GM$. But  $R[r,v]$ does not lie in $\GM$. In fact, by construction, $R[r,v]$ does not contain any edge of $\GM$. Thus, $R[r,v]$ is the shortest path from $r$ to $v$ avoiding edges of $\GM$, that is $R[s,v] = d(r,v,\GM)$.

%Since we have added the edges $X$ to $\GM$, we have added an edge from $r \to v$ with weight $d(r,v,\GM)$. Thus, there is a path in $\GM \cup X$ that avoids $\FF$ and has length $|R|$.





    \item $R$ visits an edge of $\GN$ and then merges with $\PP$ (See  \Cref{fig:gmgm}(a))

    %In this case, we will prove that $|st \DIA e| = |sr \DIA e| + |rt|$. To this end, let us first prove that $R$ merges with $\PP$ at $r$.

    In this case, we will show that $R$ merges with $\PP$ at $r$. For contradiction, let $w$ be the  vertex at which $R$ merges with $\PP$  such that $w  \neq r$.
 Let $u$ be the first vertex of $\GN$ visited by $R$.
  Also, $w$ lies after $u$ on path $R$. Thus, the replacement path $R = R[s,u]+ R[u,w] + R[w,t]$.  Since $w$ lies below $e$ on $\PP$, $wu$ sub-path of $su$ does not contain $e$ and is also the shortest path from $w$ to $u$. Thus, $R[u,w] = uw$. But $uw$ path passes through $r$. This implies that $R$ merges with $\PP$ at $r$ contradicting our assumption that $w \neq r$.
\end{enumerate}

\end{proof}

 We are now ready to prove the main lemma in this subsection.

\begin{lemma}
\label{lem:ste}
Let $e \in \PP$ and   $t \in \GM$. Assume that   the jumping replacement path $R =st \DIA e$ uses some edges of $\GN$. Then $|st \DIA e| = |sr \DIA e| + |rt|$.
\end{lemma}

\begin{proof}
Using  \Cref{lem:passr}, $R$ passes through $r$. So, we have $R = R[s,r]+ R[r,t]$. The first  summand on the right hand side of the above equality represent a path from $s$ to $r$ avoiding $e$. Thus, $|R[s,r]| = |sr \DIA e|$.

We will now show that $|R[r,t]| = |rt|$. Clearly $|R[r,t]| \ge |rt|$ as the first path avoid $e$ and the second path may or may not. We will now show that the second path also avoids $e$ which will imply that both paths are of same length.  For contradiction, assume that $rt$ passes through $e$. Let us assume that there is a vertex $w$ before the edge $e$ on path $\PP$  such that $rt = rw + wt$. Thus,  $rw$ passes through $e$  but $wt$ avoids $e$. But then, there is a path $R'$ such that $R' = sw + wt$ which avoids $e$. We claim that $|R'| < |R|$ contradicting the fact that $R$ is the replacement path from $s$ to $t$ avoiding $e$.

To this end,
\begin{tabbing}
\hspace{30mm}$|R|$\= $= |sr \DIA e| + |R[r,t]|$\\
\>$\ge |sr \DIA e| + |rt|$\\
\>$=  |sr \DIA e|  + |rw| + |wt|$\\
\> $\ge |sr \DIA e|+|wt|$\\
Since $|sw| < |sr|$, $|sw| < |sr \DIA e|$\\
\>$> |sw| + |wt|$\\

\>$= |R'|$.
\end{tabbing}
\
This completes the proof of the lemma.
\end{proof}


%\end{enumerate}

\subsubsection{$e \notin \PP$ }
\label{sec:gmgnnp}
In this case, we will show a path in $\GM \cup X$ such that it avoids $e$ and has the same length as $st \DIA e$. Please see  \Cref{fig:gmgm}(b) for a visualization of this case.

\begin{lemma}
\label{lem:enotinP}
Let $e \in \GM \SM \PP$ and   $t \in \GM$. Assume that   the replacement path $R =st \DIA e$ uses some edges of $\GN$. Then there is a path in $\GM \cup X$ that avoids $e$ and has length $|st \DIA e|$.
%be jumping. If $R$ uses some edges of $\GN$ then it passes through $r$. Moreover, $|R| = |sr \DIA e| + |rt|$
\end{lemma}
\begin{proof}
%Since $R$ is jumping, it merges back to $\PP$. There are two ways in which this can happen:
Let us first prove that  $R$ can alternate between edges of $\GN$ and $\GM$ just once. To this end,  let   $u $ be the last vertex of $\GN$ visited by $R$. Thus, $R = R[s,u] + R[u,t]$. But the shortest path $su$ remains intact in $\GG \setminus e$ as $e \notin \PP$ and the shortest $su$ path passes through $r$. This implies that $R = R[s,u] + R[u,t] = R[s,r] +\ R[r,u] +\ R[u,t]$. By construction, the first path $R[s,r] = sr$ and it completely lies in $\GM$. The second path $R[r,u]=ru$ and it completely lies in $\GN$. Let $v$ be the vertex just after $u$ in $R$. So, $v \in \GM$. So we have $R =sr +\ ru +\ (u,v)+R[v,t]$. By construction,  $R[v,t]$ completely lies in $\GM$. Thus, $R$ alternates from edges of $\GN$ to $\GM$\ just once.

From the above discussion $R = R[s,r] + R[r,u] + (u,v) + R[v,t] = R[s,r] + R[r,v]+ R[v,t]$.   The first and the last paths of the above equality completely lies in $\GM$. By construction, $R[r,v]$ does not contain any edge of $\GM$. Thus, $R[r,v]$ is the shortest path from $r$ to $v$ avoiding edges of $\GM$, that is $|R[r,v]| =|rv \DIA \GM| = d(r,v,\GM)$.

Since  we have added an edge from $r$ to $v$ with weight $d(r,v,\GM)$, we will now show that there is a path in $\GM \cup X$ that avoids $e$ and has same weight as $R$. Consider the path $R' = R[s,r] + (r,v) + R[v,t]$. The reader can check all the three subpaths lie completely in $\GM \cup X$. Moreover, $(r,v) \in X$ is a weighted edge. Thus the weight of $|R'|  =|R[s,r]| + wt_{(\GM\cup X)}(r,v)+|R[v,t]| =|R[s,r]| + d(r,v,\GM)+|R[v,t]|=|R[s,r]| + |R[r,v]|+|R[v,t]|=|R|$. 
 This completes the proof.


%If $R$ uses vertex from $N$ after it gets back to $P$, then to go into $N$ it must use $r$ as it will b in the shortest path. If it uses vertex from %$N$ before getting back to $P$, then from that path to return to $P$ it must %use $r$ as that is the shortest path and is part of BFS.


\end{proof}


\subsection{$e \in \GN$ and $t \in \GM$}
\label{sec:gngm}
In this case, $st$ path completely lies in $\GM$ and thus survives. Thus, $|st \DIA e| = |st| = d(s,t)$.


\subsection{$e \in \GN$ and $t \in \GN$}
\label{subsec:NN}

In this case, we will recurse in $\GN$. However, $\GN$ may not contain the source $s$ if $s \neq r$. In that case, before recursing, we add a new source $s_{\NN}$ in $ \GN$.
We also  add some {\em weighted }edges to $\GN$. For each $v \in \GN$, we add an edge from $s_{\NN}$ to $v$ with a weight $d(s,v,\GN) = |sv \DIA \GN| $.  Let this set of edges be called $Y$.
Let us now show that we will find all the replacement paths if we recurse in $\GN \cup Y$.

\begin{lemma}
\label{lem:4.4}
Let $e \in \GN$ and $t \in \GN$. There is a path from $s_{\NN}$ to $t$ in $\GN \cup Y$   that avoids $e$ and has weight $|st \DIA e| $.
\end{lemma}
\begin{proof}
\label{GNPath}


Let $R =st \DIA e$.
Let us first prove that once  $R$ visits an edge of  $\GN$, it cannot visit an edge of $\GM$ anymore. Let $u$ be the last vertex of $\GM$ visited by $R$ and $v$ be the vertex after $u$ in $R$. Thus, $v \in \GN$.  Thus, $R = R[s,u] +(u,v)+ R[v,t]$. By construction, $R[v,t]$ completely lies in $\GN$. The shortest path $su$ remains intact in $\GG \setminus e$ as $e \in \GN$ and the path $su$ completely lies in $\GM$. Thus, $R[s,u] = su$ . So, the path $R$ first visits only edges of $\GM$(in $R[s,u])$, then goes to $\GN$ (by taking the edge $(u,v)$) and then remains in $\GN$ (in $R[v,t]$). Thus, $R$ does not visit any edge of  $\GM$ once it visits an edge of $\GN$.

%There are two
%Let us assume that $st \DIA e$ passes through $r$. In that case, $|st \DIA e| = |sr| + |rt \DIA e|$. Thus, there is a path $rt \DIA e$ is $\GN$ of size $|st \DIA e| - |sr|$. Let us now assume that $R = st \DIA e$ does not pass through $r$.
By the above discussion,  $R = R[s,u] +\ (u,v)  + R[v,t] = R[s,v] +R[v,t]$ such that   $R[v,t]$  completely lies  in $\GN$. Also,  $R[s,v]$ completely lies in $\GM$ except the last edge which has one endpoint in $\GM$ and other endpoint $v \in \GN$. %This implies that $R[s,v]$ is the shortest path from $s$ to $v$ avoiding all edges of $\GN$. 
Thus, $R[s,v] = |sv \DIA \GN|= d(s,v,\GN)$ and we have $R =  sv \DIA \GN +\ R[v,t]$.

Now consider a path $R'$ that avoids $e$ from $s_{\NN}$ to $t$ in  $\GN \cup Y$. We construct this path as follows: we will first take the weighted edge $s_{\NN} \to v$ and then the path $R[v,t]$. The reader can check that these two subpaths completely lie in  $\GN \cup Y$. The weight of this path is  $|R'| = |sv \DIA \GN|  + |R[v,t]| = d(s,v,\GN)  + |R[v,t]|=|R[s,v] |\ +\ |R[v,t]|= |R| $.


\end{proof}

%Using the above lemma, if we recurse in the graph $\GN \cup Y$, we will find all replacement paths that satisfy the conditions of this case.

\subsection{One endpoint of $e$ is in $\GM$ and the other is in $\GN$ and $t \in \GG$}
\label{sec:middle}
This is an easy case as the $st$ path survives in $\GG \SM e$ as $st$ does not contain $e$. Thus, $st \DIA e = st$.



%\todo{Why the recursion works. As it contains weighted edges?}


==> deleted.tex <==

\subsection{Detour point on $sa$ path and merging point on $td$ path}
\label{satd}

We start this section by describing the data structures used in this section.

\begin{enumerate}
        \item $\DD^2_{nn}(s,t,l_1,l_2) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ among all $(e_1,e_2)$ pairs such that the distance $l_1$ from $s$ on the primary path and  $l_2$ from $t$ on secondary path is intact. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD^2_{nn}(s,t,l_1,l_2) $.
        
        \item $\DD^2_{fn}(s,t,p,l_2) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ among all $(e_1,e_2)$ pairs such that the replacement path avoiding $(e_1,e_2)$ from $s$ to $t$ passes through $s$-free vertex $p$ (i.e. no fault on $sp$ path or $T_s(p)$ subtree) and $l_2$ distance from $t$ on secondary path is intact from faults. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD^2_{nf}(s,t,p,l_2) $.      
        
        \item $\DD^2_{nf}(s,t,l_1,q) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ among all $(e_1,e_2)$ pairs such that the replacement path avoiding $(e_1,e_2)$ from $s$ to $t$ passes through $t$-free vertex $q$ (i.e. no fault on $tq$ path or $T_t(q)$ subtree) and $l_1$ distance from $s$ on primary path is intact from faults. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD^2_{nf}(s,t,l_1,q) $.         
         
 \todo{Next one is same as previous section}
        \item $\DD_{ff}(s,t,p,q) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ among all $(e_1,e_2)$ pair such that the replacement path from $st \diamond \{e_1,e_2\}$ passes through $s$-free vertex (i.e. no fault on $sp$ path or $T_s(p)$ subtree) $p$ and $t$-free vertex $q$. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{ff}(s,t,p,q) $.
        
   \end{enumerate}

We describe our algorithm in this case.
\todo{Should we ommit next section of paragraph?}
 Note that, at any point of time if our fault set $\{e_1,e_2\}$ satisfies the condition given in the maximiser and the maximising path does not pass through any one of the edges, then the path $st \diamond \{e_1,e_2\}$ is the path from $s$ to $t$ avoiding the maximising pair and as we store the replacement path corresponding to the maximising pair, we can just return the path.

At first, we call $\DD^2_{nn}(s,t,d_1,d_2) $ where $d_1=|se_1|$ and $d_2=|te_2|$. We can assume that, at least one of the maximising pair lies on the path, $P$. Let $x$ be a point that lies at the intersection of $P$ and the maximizing pair.. Here, we claim that, either $x$ is an intermediate vertex (i.e. $sx$ and $tx$ has some faults) or it is $s$-free vertex or $t$-free vertex. 

If $x$ is a $s$-free vertex, then we call $\DD^2_{fn}(s,t,x,d_2) $ where $d_2=|te_2|$. Then, either we get the path itself by the data structure, or we get some intersecting vertex, $y$ with the path $P$ and the maximising pair. In the later case, $y$ is a $t$-free vertex or an intermediate vertex. If it is an intermediate vertex, then we simply recurse. Else, we call $\DD_{ff}(s,t,x,y) $ which either gives us the path $P$ or an intermediate vertex. Then, we recurse on both the parts. The case if $x$ is a $t$-free vertex can be handled similarly.

\begin{algorithm}
\caption{ $\QFT_1 (s,t,F,r) $  Query Algorithm for $|st \diamond F |$ where $F=\{ e_1,e_2 \}$, $r=|F|$ in case \ref{satd} }

\If{$st \cap F \neq \phi $} 
   {
   $d_1=|se_1|,d_2=|te_2|$\;
   $(M,L) \leftarrow \DD^2_{nn}(s,t,d_1,d_2)$ \tcc*{ $M$ is edge set returned and $L$ is length of path returned }
   $\AN= L$\  \tcc*{If maximising pair does not intersects with P}
   
   \For{ $x$ in $V(M)$}
     {
      \If{$sx \cap F \neq \phi $ and $tx \cap F \neq \phi$} 
      { $\AN= \min \{\AN, \QFT_1 (s,x,F,r-1)+\QFT_1 (x,t,F,r-1) \} $\; 
      
      }
      
      \If{$sx \cap F = \phi $ \tcc*{ $x$ is $s$- free }}
       {
       $d_2=|te_2|$\;
       $(N,L) \leftarrow \DD^2_{fn}(s,t,x,d_2)$\;
       $\AN = \min \{ \AN, L \}$ \;
       
       \For{ $y$ in $V(N)$}
       {
       \If{$ty \cap F \neq \phi $}
       { $\AN= \min \{\AN, \QFT_1 (s,y,F,r-1)+\QFT_1 (y,t,F,r-1) \}$ 
       
       }
       \Else{$(O,L) \leftarrow \DD_{ff}(s,t,x,y) $\;
       $\AN = \min \{ \AN, L \}$ \;
       
       \For{ $z$ in $V(O)$} 
       {
        $\AN= \min \{\AN, \QFT_1 (s,z,F,r-1)+\QFT_1 (z,t,F,r-1) \}$ \;
        
       }
       
       }
       
       
       }
       
        }
        
        
        \If{$tx \cap F = \phi $ \tcc*{ $x$ is $t$- free }}
       {
       $d_1=|se_1|$\;
       $(N,L) \leftarrow \DD^2_{nf}(s,t,d_1,x)$\;
       $\AN = \min \{ \AN, L \}$ \;
       
       \For{ $y$ in $V(N)$}
       {
       \If{$sy \cap F \neq \phi $}
       { $\AN= \min \{\AN, \QFT_1 (s,y,F,r-1)+\QFT_1 (y,t,F,r-1) \}$ 
       
       }
       \Else{$(O,L) \leftarrow \DD_{ff}(s,t,y,x) $\;
       $\AN = \min \{ \AN, L \}$ \;
       
       \For{ $z$ in $V(O)$} 
       {
        $\AN= \min \{\AN, \QFT_1 (s,z,F,r-1)+\QFT_1 (z,t,F,r-1) \}$ \;
        
       }
       
       }
       
       
       }
       
        }
     }
   }

\Else
   {\textbf{return} |st|\;}

\textbf{return} \AN \;

\end{algorithm}

\newpage



This case is similar like previous section.

\subsection{Detour point on $sc$ path and merging point on $td$ path}


\begin{algorithm}[H]
\caption{$D(s,t,F)$: Distance between $s$ and $t$ avoiding the edge $e$}

$\AN = \QFT(st,e)$\;
$d= \min\{|su|,|sv|\}$\;
%$d_2 = \min_{x \in \{u,v\}-\OU} \{|tx|\}$\;
\textbf{if} $i=0$ \textbf{then} $d = 2^{\lfloor \log  d_1 \rfloor}$\;
% \textbf{if} $j=0$ \textbf{then} $d_2 = 2^{\lfloor \log  d_2 \rfloor}$\;

 Let $e^*= \DD(st,d)$ \;

 $\AN= |st \DIA e^*|$ \tcc*{If $e^*$ is not on the path $P$}

 

 \If(\tcc*[f]{If $e^*$ is on the path $P$}){$e \neq e^*$}  {    
 Let $e^*=(p,q)$\; 

        Let us assume that $|sp| \le |sq|$ and $|su| \le |sv|$\;
        \If{$|sp| \ge . |su|$ }
        {
                $\AN =  \min\{\AN, |sp| + \QFT(pt,e)\}$\;
  }
  \Else
  {
   \tcp{In this case $i$ will be equal to 0}

                Let $k = \lfloor \log |sp| \rfloor$\;
                Let $r \in \LL_k$ be the nearest vertex to $p$ in $pt$ path \;
                $\AN=\min \{\AN, |sr| + \QU(r^kt,e)\}$\;
  }
 }
 
\textbf{return} $\AN$ \;
\end{algorithm}







\subsection{Data Structures Stored}
At first, in this section we describe the data-structures stored for our oracles and size of the data-structures. 


\begin{enumerate}
        
        
        
        \item $\DD_{21}(s,t,d_1,d_2) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ such that length of $e_1^*s$ subpath of $st$ path is $d_1$, where $d_1=|se_1|$ and length of $e_2^*t$ subpath in $st \diamond e_1^* $ path is $d_2=|te_2|$. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{21}(s,t,d_1,d_2) $.
        
        \item $\DD_{22}(s,t,p,d_2) $ which stores the $(e_1^*,e_2^*)$ pair maximising the distance between $s$ and $t$ such that the replacement path from $s$ to $t$ passes through $s$-free vertex (i.e. no fault on $sp$ path or $T_s(p)$ subtree) $p$ and the length of $e_2^*t \diamond e_1^*$ subpath of $st \diamond e_1^*$ is $d_2$ from $t$ where $d_2=|te_2|$. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{12}(s,t,d_1,d_2) $.
        
        \item $\DD_{31}(s,t,l_1,l_2) $ which stores the $(e_1^*,e_2^*)$ pair which maximises the distance between $s$ and $t$ among all $(e_1,e_2)$ pair such that distance of $e_1,e_2$ from $s$ and $t$ are  $l_1$ and $l_2$ , respectively where $l_1=|se_1|,l_2=|te_2|$. We also store the path $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{31}(s,t,l_1,l_2) $.
        
   \item $\DD_{32}(s,t,j,l_1,l_2) $ which stores the $(e_1^*,e_2^*)$ pair which maximises the distance between $s$ and $t$ among all $(e_1,e_2)$ pair such that distance of the fault on $st$ path, $e_1$ is atleast $(1+\epsilon)^j$ from $s$ and the distance of the second fault $e_2$ on $st \diamond e_1$ is at least $l_1$ and $l_2$ from $s$ and $t$ respectively.
    
   \item $\DD_{33}(s,t,j,l_1,q) $ which stores the $(e_1^*,e_2^*)$ pair which maximises the distance between $s$ and $t$ among all $(e_1,e_2)$ pair such that distance of the fault on $st$ path, $e_1$ is atleast $(1+\epsilon)^j$ from $s$ ,the distance of the second fault $e_2$ on $st \diamond e_1$ is at least $l_1$ . Also, the path $st \diamond \{e_1,e_2\}$ passes through $t$-free vertex $q$.


        
\end{enumerate}

        
\subsection{Algorithm and Overview}

We divide our algorithm in some cases depending on the detour point (the first point from where detour from the shortest path starts) and merging point (the point after which the replacement path and shortest path are same) of the replacement path, $P$. Also, for the cases below we assume that only $e_1=(a,b)$ is on the shortest $st$ path.
\todo{Shoould we replace $sc,td$ and so on by $se_1, te_2$ and so on?}

\textbf{Case 1: Detour point on shortest $sa$ path and merging point on shortest $tb$ path : }
 
  
  
  \textbf{Case 2: Detour point on shortest $sa$ path and merging point on shortest $td$ path :} 
  In this case, we call $\DD_{21}(s,t,d_1,d_2) $ and get the maximising pair $(e_1^*,e_2^*)$. If both the edges does not lie on $P$ then the path returned by the data structure $ \PP \DD_{21}(s,t,d_1,d_2) $is our desired path.
  
 Else, let $e_1^*=(x,y)$ be the edge intersecting with $P$. Then, it can be shown that, the vertex $x$ is $s-$ free and hence, can act as a helper vertex. Now, we can call the data structure $\DD_{22}(s,t,x,d_2) $. Similar like previous, we if both the edges does not lie on $P$ then the path returned by the data structure $ \PP \DD_{22}(s,t,x,d_2) $is our desired path. Else, we get some vertex $y$ on the path $P$ which is $t$-free. 
 
 After this, we call $\DD_H(s,t,x,y) $ and either get the path from $\PP \DD_H(s,t,x,y) $ if the maximising pair not intersecting with path $P$ or, get the hitting element $z$. This way, we get the hitting element and recurse the same process to get both subpaths, $sz \diamond \{e_1,e_2\}$ and $zt \diamond \{e_1,e_2\}$.
  
Similarly, the case if $e_2^*=(x,y)$ is the edge intersecting with $P$ can be handled similarly like before as then $x$ will be $t$-free and so on.
 
   \textbf{Case 3: Detour point on shortest $sc$ path and merging point on shortest $tb$ path :}
   This case is similiar to Case 2. In this case, we can swap $s$ and $t$ from  previous case and get the problem solved like previous one.
   
   \textbf{Case 4: Detour point on shortest $sc$ path and merging point on shortest $td$ path :}
   We divide this case into 4 subcase depending on the lengths of $sa,sc,tb,td$. 
   
   \textbf{Subcase 4.1: $|sa| < |sc|$ and $|td| \leq |tb|$ :} Let, the distance be $|sa|=d_1$ and $|td|=d_2$. Next, we call the data structure $\DD_{31}(s,t,d_1,d_2)$ and get the maximising pair $(e_1^*,e_2^*)$. If both the edges does not lie on $P$ then the path returned by the data structure $ \PP \DD_{21}(s,t,d_1,d_2) $ is our desired path. If it intersects with path $P$ and the intersecting vertex is nearer to $t$ on path $P$ then we can show that this is a $t$-free vertex. Else, we may or may not get a $s$-free vertex if the vertex is nearer to $s$ in $P$. If we get the vertex nearer to $s$, depending on whether or not it is a $s$-free vertex we can divide it into further subcases.
   
   \textbf{Subsubcase 4.1.1: The intersecting vertex, $p$ is not a $s$-free vertex : } In this case, $p$ has to be on the shortest $sc$ path. Now, we have to find the path from $p$ to $t$ avoiding $f_1,f_2$. Also, note that the shortest path $sp$ is undisturbed. We further divide into two cases depending on which edge among $f_1$ and $f_2$ is closer to $p$.
   
   \textbf{Subsubsubcase 4.1.1.1: If $f_1$ is closer to $p$ : } In this case, we can say that, the point $a$ will be outside the trapezoid of the path $P[p,t]$. Now, if $l$ is the LCA of $a,c$ in $T_p$ then, there will be some $i$ such that $(1+\epsilon)^{i} > |pl| > (1+\epsilon)^{i-1}$ and $|pa| > (1+\epsilon)^{i}$. In this case, we call the data structure $\DD_{32}(p,t,i,d_1,d_2)$ where $d_1=|pc|, d_2=|td|$. Now, if the intersecting vertex is nearer to $p$ then we get a $p$-free vertex which is also $s$- free and can act as helper vertex. If not, then we get a $t$-free vertex $q$. Then we call the data-structure $\DD_{33}(s,t,j,d_1,q)$. If it intersects with $P$ then we get another vertex which is $s$- free. After that, we call $\DD_H(s,t,p,q)$ to either get the path as $\PP \DD_H(s,t,p,q)$ or get a hitting element.
   
   \textbf{Subsubsubcase 4.1.1.2: If $f_2$ is closer to $p$ : } In this case, we call $\DD_{11}(p,t,d_1,d_2)$ where $d_1=|pc|$ and $d_2=|td|$. Now, if the maximising pair intersects with path $P$ then we get either a $p$-free or $t$-free vertex and similar like previous cases we get another helping vertex and get a hitting element in next attempt.
   
  \textbf{Subsubcase 4.1.1: The intersecting vertex, $p$ is a $s$-free vertex : } In that case, we get a helper vertex and then similarly like before, we get another helper vertex from which is $t$-free and then get a hitting element.
  
  This concludes subcase 4.1. The other subcases can be done in similar way.


  
\newpage
\begin{algorithm}[H]
\caption{$D(s,t,F)$: Distance between $s$ and $t$ avoiding the edge $e$}

$\AN = \QFT(st,e)$\;
$d= \min\{|su|,|sv|\}$\;
%$d_2 = \min_{x \in \{u,v\}-\OU} \{|tx|\}$\;
\textbf{if} $i=0$ \textbf{then} $d = 2^{\lfloor \log  d_1 \rfloor}$\;
% \textbf{if} $j=0$ \textbf{then} $d_2 = 2^{\lfloor \log  d_2 \rfloor}$\;

 Let $e^*= \DD(st,d)$ \;

 $\AN= |st \DIA e^*|$ \tcc*{If $e^*$ is not on the path $P$}

 

 \If(\tcc*[f]{If $e^*$ is on the path $P$}){$e \neq e^*$}  {    
 Let $e^*=(p,q)$\; 

        Let us assume that $|sp| \le |sq|$ and $|su| \le |sv|$\;
        \If{$|sp| \ge . |su|$ }
        {
                $\AN =  \min\{\AN, |sp| + \QFT(pt,e)\}$\;
  }
  \Else
  {
   \tcp{In this case $i$ will be equal to 0}

                Let $k = \lfloor \log |sp| \rfloor$\;
                Let $r \in \LL_k$ be the nearest vertex to $p$ in $pt$ path \;
                $\AN=\min \{\AN, |sr| + \QU(r^kt,e)\}$\;
  }
 }
 




\textbf{return} $\AN$ \;
\end{algorithm}


\todo{But then we could directly use $FT(x_1,v)?$}
 \subsection{Query Time}
 
 




==> departing.tex <==


\section{Departing Replacement paths}
\label{sec:departing}

In the previous section, we have already found out a replacement path if it is jumping or if the edge failure is not on the primary path. In this section, we will try to find the best departing path after an edge failure. To this end, we define the following:
\begin{definition} (Candidate departing paths)
Let $e \in \PP$. $P$ is called the candidate departing path for $e$, if among all departing paths avoiding $e$, $P$ has the minimum length. In case there are many departing paths avoiding same edge with same length, we will break ties using Definition \ref{def:replacementpath}.
\end{definition}

Note that, a candidate departing path may or may not be a replacement path. In case it is, we call it a departing replacement path. Also, $P$ may be a candidate departing path for all edges in an interval, say $yz \in \PP$, but may be a replacement path for a sub-interval of $yz$.
With this definition in hand, we will now find all candidate departing paths.

\subsection{Finding all candidate departing paths}

In the previous section,  we added some weighted edges in the graph when we recurse. Thus, there might be two types of edges in the graph -- {\em weighted}  and {\em unweighted}. The weighted edges represent paths in the graph $\GG$, and the unweighted edges are present in $\GG$. $\GG$ contains only unweighted edges. However, the graph at an internal node of $\TTT$, say graph $\GAT$, may have weighted as well as unweighted edges.

In the ensuing discussion, let $\GAT$ be the graph processed by our algorithm at some internal node of $\TTT$. In the graph $\GAT$, we will assume that there is a source $s$. Let $\overline{\GG}$ be the parent of  $\GAT$.  In our algorithm, we partition $\overline{\GG}$ into two disjoint graphs and then recurse on it. If  $\GAT$ is the left child of $\overline{\GG}$, then it includes a set  $X$  of weighted edges added by us in  \Cref{subsec:MM}. Similarly, if $\GAT$ is the right child of $\overline{\GG}$ then it includes a set  $Y$  of weighted edges added by us in  \Cref{subsec:NN}. Using the separator lemma, we will find the vertex $r$ that  partitions $\BFS_{\GAT}(s)$ . Also, the primary path $\PP = sr$.

We now give an overview of our method to find candidate departing paths in $\GAT$. To this end, we will use the main idea in the paper of Gupta and Singh \cite{GuptaS18}.  In \cite{GuptaS18}, the authors proved \Cref{lem:guptaaditi}.
Though they did not mention it, the paths in the \Cref{lem:guptaaditi} look very much like the departing paths. Indeed, that lemma is more general than what the authors originally intended it to be. The authors show the above lemma for a specific vertex $t_s$, but a careful reading of the paper suggests that the above lemma is true for any vertex on the $st$ path. We now generalise this lemma.
However, there is one problem. The above result holds only for an unweighted graph, whereas $\GAT$ is weighted. Thus, we cannot prove the above lemma as it is. However, we will prove the following weaker lemma:

\begin{lemma}
\label{lem:guptaadapted}
Let $\GAT$ be the graph at  an internal node in the binary tree $\TTT$. Let $s$ be the source of $\GAT$. For a destination $t \in \GAT$, let $p$ be any vertex  on $st$ path. The number of replacement paths from $s$ to $t$ that avoid edges on $sp$ path  and also avoid  $p$ is $O(\sqrt n)$.
\end{lemma}

Some discussion is in order. In an ideal case, the number of replacement paths that avoid edges on $sp$ and also avoid $p$ should have been $\OO(\sqrt {n_{\GAT}})$. This result would have been similar to  \Cref{lem:guptaaditi}. Unfortunately, we cannot prove this result as $\GAT$ is weighted. However, if we just expand the weighted edge in the graph $\GAT$, then  we will get an unweighted graph. By expanding, we mean that for each weighted edge, add the path that represents that weighted edge. However, this process  may increase the number of vertices in the graph to $n$. Now, we can adapt   \Cref{lem:guptaaditi}. For an unweighted graph with $n$ vertices, this lemma guarantees that the number of replacement paths avoiding $p$ will be at most $\sqrt n$. Indeed, this is our result in  \Cref{lem:guptaadapted}. We prove this lemma in \Cref{adapted} as it is an extension of the proof in \cite{GuptaS18}.

 \Cref{lem:guptaadapted} implies that there are only $O(\sqrt n)$ replacement paths that have some special properties which are similar to the properties of departing paths.
So, our plan of action is as follows:

\begin{enumerate}
    \item Show that there are only $O(\sqrt n)$ candidate departing paths to $t$ in $\GAT$. This will be done by showing the similarity between the replacement paths in  \Cref{lem:guptaadapted} and candidate departing paths.

    \item Show that we can find the lengths of all the candidate departing paths in $\GAT$ in  $O(m_{\GAT} \sqrt n)$ time. Additionally, we show that we can store the lengths	 in a compact data structure of size $O(n_{\GAT}\sqrt n)$.  Given any query $\QU(s,t,e)$ to this data-structure such that $s,t \in \GAT$ and $e$ is on the primary path of $\GAT$, we can find the length of  corresponding candidate departing path in $\TL(1)$ time.
\end{enumerate}

This completes the overview of our algorithm for finding candidate departing paths.

\subsection{Similarity between candidate departing paths and replacement paths in  \Cref{lem:guptaadapted}}

 Let us first prove some simple results that will help us prove this section's main idea.
\begin{lemma}
\label{lem:departingproperty}
Let $t \in \GT$ and $p = \LCA(t,r)$. All the candidate departing paths from $s$ to $t$ avoiding edges on $sp$ path also avoid $p$. For any edge $e$ on $pr$ path , $st \DIA e = st$. %Thus, this replacement path passes through $p$, since $st = sp+pt$.
\end{lemma}

\begin{proof}
Let $R = st  \DIA e$ where $e \in sp$ and $R$ is departing.  The detour of $R$ must start above $e$ on $\PP$.  Since $R$ is departing, it can not merge with the path $\PP$ again. So, it avoids $p$ also.

The $st$ path passes through $p$ and does not use any vertex of $\PP$ below $p$. So, removing any edge on $pr$ path  does not disturb $st$ path. So, for any edge $e \in pr$ , $st \DIA e = st$.




\end{proof}

We now show that the candidate departing paths and the replacement paths in  \Cref{lem:guptaadapted} have the same property.
%We will then  use this similarity and  the power of Lemma \Cref{lem:guptaadapted} to prove the following lemma:

\begin{lemma}
\label{lem:numberofdeparted}
For any vertex $t \in \GAT$, there are $\OO(\sqrt{n})$ candidate departing paths to $t$.
\end{lemma}
\begin{proof}
 \label{cdpnumbers}
 Remember that the candidate departing path avoids edges on path $\PP$ only. Let $p = \LCA(r,t)$. Using  \Cref{lem:departingproperty}, $st$ is the candidate departing path avoiding all edges in $pr$ path. Again, by  \Cref{lem:departingproperty}, all the candidate departing paths avoiding edges in $sp$ path  avoid $p$ too. But by  \Cref{lem:guptaadapted}, the number of such paths is $O(\sqrt n)$. This implies that there are $O(\sqrt n)$ candidate departing paths to $t$.

\end{proof}

Given the above lemma, we need to store $O(\sqrt n)$ candidate departing paths to $t$ in $\GAT$. Before designing an algorithm to find candidate departing paths, we first see how we plan to store these paths in a compact data structure.


\subsection{The data-structure at each node of $\TT$}
Let us first discuss a small technical detail that may be perceived as a problem but is not. Our graph $\GAT$ is weighted. It stands to reason that even the primary path $\PP$ in $\GAT$ maybe weighted. Since candidate departing paths are only for the faults on the primary path, it may not be clear what happens if the edge on the primary path is weighted. To this end, we show that on any $st$ path in $\GAT$, all edges except may be the first one, are unweighted.

\begin{lemma}
\label{lem:dsatT}
For $t \in \GAT$, except may be the first edge of $(st)_\GAT$, all other edges of $(st)_\GAT$ are unweighted.
\end{lemma}

\begin{proof}
   \label{structure}
  We will prove using induction on the nodes of $\TT$. In the root of $\TTT$, we have the graph $\GG$. Clearly, the graph $\GG$ satisfies the property of the lemma. Let us assume using induction that the parent of the graph $\GAT$ satisfies the property of the lemma. Let $\overline{\GG}$ be the parent of $\GAT$. Let $\overline{s}$ be the source in $\overline{\GG}$. Thus, in the graph $\overline{\GG}$, using the separator lemma, we find a $\overline{r}$ that divides $\overline{\GG}$ into two parts. The path from $\overline{s}$ to $\overline{r}$, say $\overline{\PP}$ is the primary path. By induction, only the first edge of the primary path may be weighted.  There are two cases:

\begin{enumerate}
\item $\GAT$ is the left child of $\overline{\GG}$.

In this case, the source of $\GAT$ is also $\overline{s}$.
For each $t \in \GAT$, it can be observed  that the path $(\overline{s}t)_{\overline{\GG}} = (\overline{s}t)_\GAT$. Using induction hypothesis, since $(\overline{s}t)_{\overline{\GG}}$ satisfies the statement of lemma, so does $(\overline{s}t)_\GAT$.
\item $\GAT$ is the right child of $\overline{\GG}$.

There are two cases. When $\overline{s} = \overline{r}$, then we fall back in point(1). So, let us look at the case when $\overline{s} \neq \overline{r}$.

For a $t \in \GAT$, by construction, $(\overline{s}t)_{\overline{\GG}}$ passes through $\overline{r}$. Thus, $(\overline{s}t)_{\overline{\GG}} = (\bar{s}\bar{r})_{\overline{\GG}} + (\overline{r}t)_{\overline{\GG}}$. In $\GAT$, we add a new source $s$. Also, we add a weighted edge  from $s$ to $\overline{r}$ in $\GAT$.  The weight of this edge is $|\bar{s}\bar{r} \DIA \GAT|_{\overline{\GG}}$. Also, $(\overline{r}t)_{\overline{\GG}} = (\overline{r}t)_\GAT$. This implies that there is path in $\GAT$ from $s$ to $t$, $(s,\overline{r})+ (\overline{r}t)_\GAT$. By induction, we claim that on this path except $(s,\overline{r})$, all the edges are unweighted.
\end{enumerate}

\end{proof}



Using the above lemma, all except the first edge of the primary path are unweighted. The weighted edges represent edges for which we have already found candidate departing paths at the parent or an ancestor of $\GAT$. Thus, we will only find candidate departing paths for unweighted edges in $\PP$.  In the ensuing discussion, whenever we mention a path avoiding an edge on the primary path, it will always refer to an unweighted edge.

 We now prove some simple lemmas that will help us build data structures for candidate departing paths.
\begin{lemma}
\label{lem:reldeparting1}
Let $R$ and $R'$ be two different candidate departing paths from $s$ to $t$ avoiding edges $e$ and $e'$  respectively on the path $\PP$. If $e$ lies above  $ e'$ on $\PP$, then $|R|>|R'|$.
\end{lemma}
\begin{proof}
The detour of the candidate departing $R$ starts before $e$, and once it departs, it does not merge with $\PP$ again.  As $e$ lies above  $e'$ on $\PP$, $R$  also avoids $e'$. If $|R| \leq |R'|$, then by \Cref{def:replacementpath}, $R$ must be  the  candidate departing path avoiding $e'$, leading to a contradiction. So, it must be the case that $|R|>|R'|$.
\end{proof}

\begin{lemma}
\label{lem:reldeparting2}
Let $R$ be a candidate departing path. Let $yz$ be the maximal subpath of $\PP$ such that $R$ is the candidate departing path for edges in $yz$. Then $\DP(R) = y$.	
\end{lemma}

\begin{proof}
\label{app:reldeparting2}
Since $R$ avoids the edges of $yz$, its detour starts at or above $y$ on the path $\PP$. Let us assume that $\DP(R)$ lies above $y$ on path $\PP$, say at $x$. This implies that $R$ also avoids all edges on $xy$ path. But $R$ is not the candidate departing path for edges in the path $xy$. Let $R'$ be the candidate departing path for an edge, say $e' \in xy$. Now, for an edge $e \in yz$, $R$ is the replacement path and $e'$ lies above $e$ on $\PP$. Using  \Cref{lem:reldeparting1}, $|R'| > |R|$. But in that case, $R$ should be the replacement path avoiding  $e'$ too. This leads to a contradiction. Thus, our assumption that $\DP(R)$ lies above $y$ is false and $\DP(R) = y$.
\end{proof}

\label{app:reldeparting3}



The above lemma states that if $R$ avoids edges in $yz$, then the detour of $R$ necessarily starts from $y$.
  We will now prove the contrapositive of the  \Cref{lem:reldeparting1}.

  \begin{lemma}
  \label{lem:reldeparting3}
Let $R$ and $R'$ be two different candidate departing paths from $s$ to $t$. If $|R|>|R'|$, then $\DP(R)$ lies above $\DP(R')$ on $\PP$.
\end{lemma}


\begin{proof}
Since $R'$ does not merge with $\PP$, $R'$ avoids all edges below $\DP(R')$ in $\PP$. Assume for contradiction, that $\DP(R')$ lies above $\DP(R)$.  This will imply that $R'$ also avoids all the edges avoided by $R$. But $|R| > |R'|$. Then, $R'$ should be the  candidate departing path for all the edges avoided by $R$ -- a contradiction. Thus, $\DP(R)$ lies above $\DP(R')$ on $\PP$.
\end{proof}

 We will now use the above lemmas and our deduction to build a compact data-structure for all candidate departing paths. To this end, we will store an array $\DEP(t)$ for each $t \in \GAT$. $\DEP(t)$ will store candidate departing paths from $s$ to $t$  in increasing order of their lengths. By  \Cref{lem:numberofdeparted}, there are  $\OO(\sqrt n)$ such paths. let us denote them by $R_1, R_2, \dots, R_k$ where $k = O(\sqrt n)$.  For any two consecutive candidate departing paths $R_i$ and $R_{i+1}$, using  \Cref{lem:reldeparting3} and \Cref{lem:reldeparting2}, we claim that $R_{i+1}$ is the candidate departing path avoiding edges in $[\DP(R_{i+1}),\DP(R_{i})]$ on the primary path $\PP$.
Since the size of $\DEP(t) = O(\sqrt n)$, the total size of $\DEP$ data-structure is bounded by $\OO(n_\GAT \sqrt n)$.


\begin{lemma}
$\sum_{t \in \GAT} \text{size of $\DEP(t)$} = O(n_\GAT\sqrt n)$
\end{lemma}
\subsection{Finding and storing all candidate departing paths efficiently}
Let us first describe the setting that will be used throughout this section. At an internal node $\GAT$ of $\TT$, we are planning to find all candidate departing paths from the source $s$. To this end, we will find a vertex $r$ that will divide $\SPT_{\GAT}(s)$ roughly equally. Also, $\PP =sr$.

To find all candidate departing path,  we will build an auxiliary graph $G$ which we will build incrementally. The source in this graph is   $(s)$. All other vertices in $G$ are tuples of the form  $(v,|R|)$, where $v \in \GAT \setminus \PP$ and $R$ is a candidate departing path to $v$.   During initialization, we will add $(v,|sv|_{\GAT})$ in $G$ for each $v \in \GAT \setminus \PP$. Also, there will be an edge from $(s)$ to $(v,|sv|_{\GAT})$ with weight $|sv|_{\GAT}$. We will show the following property at the end of our analysis.

\begin{prop}
\label{prop1}
 Let $R$ be the candidate departing path to $v$ avoiding edge on the subpath $yz$ of $\PP$.  Then, there is a vertex $(v,|R|)$ in
$G$. Moreover the shortest path from $(s)$ to $(v,|R|)$ in the graph $G$ is of length
$|R|$, that is  $|R|= |(s)(v,|R|)|_{G}$
\end{prop}

In  \Cref{lem:propertytrue}, we will show that \Cref{prop1} is true for all the nodes added during initialization. Also, we will create $\DEP(v)$ for each $v$ during intialization.
 We will store candidate departing paths in $\DEP(v)$ in increasing order of lengths. Given a departing path $R$, we will assume that we will store the following information about $R$ in $\DEP()$.
 \begin{enumerate}
\item The endpoints of $R$.
\item The weight of path $R$.
\item The last edge of $R$ and its weight.
\item $\DP(R)$.
\end{enumerate}

After initialization, we will run a variant of Dijkstra's algorithm in $G$.
To this end, we will construct a min-heap $\HH$ in which we will store all the departing paths that we have discovered at any point in the algorithm.
We use the first two points of \Cref{def:detour} to select the minimum  element from $\HH$,i.e., given two candidate departing paths $R$ and $R'$, $R$ is {\em smaller} than $R'$ if $|R| < |R'|$ or $|R| = |R'|$ and $\DEP(R)$ is closer to $s$ than $\DEP(R')$. If $\DEP(R) = \DEP(R')$, then we can break ties arbitrarily.


We now explain the adaptation of Dijkstra's algorithm. After initialization,for each $(v, |sv|)$, and for each neighbor neighbor $w$ of $v$, we add  the departing  path $sv + (v,w)$ in $\HH$ if $w \notin \PP$.
 Then, we go over all the elements of the heap till it is empty. Let us assume that $R$ is the minimum element of the heap and it ends at $v$ and $(u,v) \in \GAT$ is the last edge of $R$. This implies that $R$ was added in $\HH$ while processing a candidate departing path for $u$. Let this path be $R_u$. Thus, there is a node $(u,|R_u|)$ in $G$. We now need to decide whether $R$ is a candidate departing path for $v$.

To this end,  we look at the last candidate departing path added by us in $\DEP(v)$, let it be $Q$.  We then check if the $d_\GAT(s,\DP(R))$ is less than $d_\GAT(s,\DP(Q))$. If yes, then we have found a new candidate departing path to $v$ that avoids all edges in  $[\DP(R),\DP(Q)]$ of $\PP$. Thus, we will add the vertex $(v,|R|)$ in the graph with an edge of weight $wt_\GAT(u,v)$ from $(u,|R_u|)$. Also, for each neighbor $w$ of $v$, we will add the departing path $R+(v,w)$ to the heap if $w \notin \PP$. The pseudocode of the algorithm for finding all candidate departing path is given in algorithm 1.



\begin{algorithm}
\label{algo:cdpalgo}
\caption{Algorithm to construct $\DEP()$}


 create a vertex $(s)$\;




\For{$v \in \GAT \SM \PP$}
{


Let $R_v = |sv|_\GAT$\;   create a vertex $(v,|R_v|)$\;
   add edge between ($s)$ and $(v,|R_v|)$ with weight $|sv|_\GAT$\;
   append $R_v$ in  $\DEP(v)$\;
   \For{$(v,w) \in \GAT$ and $w \notin \PP$}
      {
      add the path $R_v+(v,w)$ in min-heap  $\HH$ \;
      }
}

\While{min-heap is non-empty}
{
  remove $R$ from the top of min-heap\;

Let us assume that $R$ ends at $v$ and the last edge of $R$ is $(u,v)$\;
Also assume that $R_u = R \SM (u,v)$ is a candidate departing path to $u$\;
  Let  $Q$ be the last candidate departing path added by us  in   $\DEP(v)$\;
  \If{$d_{\GAT}(s,\DP(R))<d_\GAT(s,\DP(Q))$}
  {
    create a vertex $(v,|R|)$\;
    add edge between $(u,|R_u|)$ and $(v,|R|)$ with weight $wt_\GAT(u,v)$ \;

    append the path $R$ in  $\DEP(v)$\;
    \For{$(v,w) \in \GAT$ and $w \notin \PP$}
    {
    add the departing path $R+(v,w)$  in min heap $\HH$\;
    }
 }

}


\end{algorithm}




\subsection{Correctness and running time of the algorithm storing candidate departing paths}
\label{subsection:correct}

We claim that, the time taken to construct the $\DEP()$ data-structure at a node of the binary tree with graph $\GAT$ is  $O(m_\GAT\sqrt n)$. Moreover, the size of the data-structure is $O(n_\GAT \sqrt n)$. In this section, we prove that  our algorithm stores correct lengths of all candidate departing paths.\begin{lemma}
	\label{lem:propertytrue}
Let $R$ be a candidate departing path to $v$ where $v \in \GAT \SM \PP$. Let $yz$ be the maximal subpath of $\PP$ such that $R$ is the candidate departing path for edges in $yz$. Then $(v,|R|) \in G$ and satisfies  \Cref{prop1}.
\end{lemma}

\begin{proof}
	We will prove the above lemma using induction on the weighted distance of a vertex from $(s)$ in $G$. During initialization, for each $v \in \GG \SM \PP$, we add a vertex $(v,|sv|_\GAT) \in G$. Also, the weight of the edge from $(s)$ to $(v,|sv|_\GAT)$ is $|sv|_\GAT$.   We claim that the statement of the lemma is true for the smallest candidate departing path to $v$. Indeed, using  \Cref{lem:departingproperty}, $(sv)_\GAT$ is the a replacement path for the edges in subpath $pr$ on $\PP$ where $p = \LCA_{\GAT}(v,r)$. Also,  $(sv)_\GAT$ is the smallest replacement path because it is the shortest path from $s$ to $v$ in $\GAT$.     Thus, the base case is true for all $v \in \GAT \SM \PP$.

Let us now assume that the statement of the lemma is true for all candidate departing paths to $v$ with length $< |R|$.  Let the second last vertex of $R$  be $u$.
Since $R$ is a candidate departing path, even $R \SM(u,v)$ is a candidate departing path. Since $R[s,u]$ has length less than $R$, by induction hypothesis, there is a vertex $(u,|R \SM(u,v)|)$ in $G$. Also there is at least one  replacement path in $\DEP(v)$  of weight less than $|R|$ -- as we have added $(sv)_\GAT$ in $\DEP(v)$. Let $Q$ be a candidate departing path of  largest weight less  than the weight of $R$. Let  us also assume that $Q$ avoids edge on subpath $zz' \in \PP$. Thus, using  \Cref{lem:reldeparting2}, $\DP(Q) = z$.  Since $|Q| < |R|$, using  \Cref{lem:reldeparting3}, $\DP(R)$ lies above $\DP(Q)$ on $\PP$.  Using the induction hypothesis,  there is a vertex $(v,|Q|)$ in $G$.

We will now show that our algorithm will add $(v,|R|)$ in $G$. There are four cases:

\begin{enumerate}
\item Our algorithm does not add any vertex for $v$ after $(v,|Q|)$

But our algorithm does process the vertex $(u,|R \SM(u,v)|)$. Thus, it will check each neighbour of $u$. When it checks the neighbor  $v$, it will  add the  departing path $R$ in the heap $\HH$. Thus, we will add the vertex $(v,|R|)$ in $G$ while processing $R$, leading to a contradiction.

\item Our algorithm adds a vertex $(v,|R'|)$ where $\DP(R)$ lies above   $\DP(R')$ on $\PP$

We claim that the weight of $R'$ cannot be less than the weight of $R$ as then  $R$ is not the candidate departing path for all the edges in $\DP(R')z$ subpath, contradicting the statement of the lemma. So let us assume that $|R| = |R'|$. But then $\DP(R)$ lies above $\DP(R')$ on $\PP$. Thus, the min-heap will give preference to the replacement path $R$ first, and our algorithm will make the vertex $(v,|R|)$. Again a contradiction.

\item Our algorithm adds a vertex $(v,|R'|)$ where $\DP(R)$ lies below  $\DP(R')$ on $\PP$

 Again, we claim that the weight of $R'$ cannot be less than the weight of $R$ as then it $R$ is not the replacement path for all edges in $yz$ subpath, contradicting the statement of the lemma. So let us assume that $|R| = |R'|$. But $\DP(R') $  is closer to $s$ than $\DP(R)$. Thus, $R'$ should be the  candidate departing path avoiding edges of $yz$. This contradicts our assumption that $R$ is the candidate departing path for all edges in $yz$.

\item Our algorithm adds a vertex $(v,|R'|)$ where $\DP(R) = \DP(R')$

$|R'|$ cannot be less than $|R|$ as otherwise our algorithm will give preference to path $R$. But, if  $|R| = |R'|$, then there is a vertex $(v, |R'|)= (v,|R|)$ in $G$. 

\end{enumerate}


So, we  add the  node $(v,|R|)$ in the graph $G$. At that moment, we also adds an edge from $(u,R\SM(u,v))$ to $(v,|R|)$ in $G$ with weight $wt_{\GAT}(u,v)$. Using induction, $|(s)(u,R\SM(u,v))|_G = |R\SM(u,v)|$. Thus, $|(s)(v,|R|)|_G = |R\SM(u,v)|\ +\ wt_\GAT(u,v) = |R|$. This completes our proof.

\end{proof}

 Let's determine the running time of our algorithm. Using \Cref{lem:numberofdeparted}, for each $v \in \GAT$, we make $O(\sqrt n)$ entries in $\DEP(v)$. In other words, we make $O(\sqrt n )$ nodes of type $(v ,\dot)$ in $G$.   Whenever we add a node $(v,|R|)$  in $G$, we see all the edges of $v$.   This implies that the total time taken to process all the vertices of $v$ in $G$ is $O( \sqrt n \deg_\GAT(v))$. Summing it over all the vertices gives us the bound of $O(m_\GAT\sqrt n)$.  Using a similar calculation, the total size of our data-structure for  $\GAT$ is $O(n_\GAT \sqrt n)$. Thus, we claim the following lemma:

\begin{lemma}
\label{lem:depconstruction}
The time taken to construct the $\DEP()$ data-structure at a node of the binary tree with graph $\GAT$ is  $O(m_\GAT\sqrt n)$. Moreover, the size of the data-structure is $O(n_\GAT \sqrt n)$.
\end{lemma}



\subsection{Querying for a candidate departing path}
\label{query}
In this section, we describe how to find a candidate departing path using our data-structure $\DEP()$. Let $t \in \GAT \SM \PP$  and $e \in \PP$ be an edge on $st$ path. Let  $st \DIA e$ be   a candidate departing path, then we can find it using  algorithm given in \Cref{app:queryCDP}.

In this algorithm, we perform a binary search in $\DEP(t)$ to find two consecutive paths $R$ and $Q$ such that $e$ lies in the interval [$\DEP(R), \DEP(Q)]$  of $\PP$. Using  \Cref{lem:reldeparting3} and \Cref{lem:reldeparting2},  $R$ is the candidate departing path avoiding $e$.
The pseudocode of the query algorithm to find the Candidate Departing path here.
\label{app:queryCDP}
\begin{algorithm}
\caption{$\QD(s,t,e)$}


%\STATE input the edge $e=(a,b)$ to be avoided and destination $t$ to be reached

 $R \xleftarrow{}$ binary search in the array of $\DEP(t)$ to find a two consecutive path $Q$ and $R$ such that $e$ lies in interval  $[\DP(R),\DP(Q)]$ of $\PP$ \;
return{ $|R|$}
\label{algo:queryd_1}
\end{algorithm}

  
\begin{algorithm}[H]
\caption{$\QU(s,t,e,\TT)$}

 $mindist \xleftarrow{} \infty $\;

  \tcc{ \Cref{sec:gmgn} }




\If{ $e \in \GM,t \in \GN $}
{
    \If{ $e \in \PP$}
    {
     \tcc{if $st \DIA e$ happens to be departing}
     $mindist \leftarrow \QD(s,t,e)$ using $\DEP()$ data-structure at $\TT$\;
     \tcc{if $st \DIA e$ happens to be jumping}

     $mindist \xleftarrow{} \min\{mindist, |sr \diamond e|+|rt|\}$
    }
    \Else{
    $mindist \leftarrow  |st|$
    }
}
\tcc{ \Cref{subsec:MM}}

\If{ $e \in \GM,t \in \GM $}
{
\tcc{ \Cref{sec:gmgmp}}
\If{ $e \in \PP $}
{
      \tcc{if $st \DIA e$ happens to be departing}
      $mindist \leftarrow \QD(s,t,e)$ using $\DEP()$ data-structure at $\TT$\;
      \tcc{if $st \DIA e$ happens to be jumping}
      $mindist \xleftarrow{} \min (mindist, |sr \DIA e|+|rt| ) $

   }
    \tcc{ \Cref{sec:gmgnnp}}
    \If{ $e \in \GM \setminus \PP $}
    {
      $mindist \xleftarrow{}  \QU(s,t,e,\text{left child of $\TT$})$
   }

}

\tcc{ \Cref{sec:gngm}}
\If{ $e \in \GN, t \in \GM $}
{z
    $mindist \leftarrow  |st|$\;
}

\tcc{ \Cref{subsec:NN}}
\If{$ e \in \GN,t \in \GN,  $}
{
   $mindist \leftarrow \QU(s,t,e,\text{right child of $\TT$}$)\;

}
\tcc{ \Cref{sec:middle}}
\If{one endpoint of $e$ is in $\GM$ and other in $\GN$}
{
$mindist \leftarrow  |st|$\;
}

return $mindist$\;
\label{alg:query}
\end{algorithm}




 \section{Construction time, size and query time of the SDO(1) } 
 In this section, we show that the construction time of our algorithm is $\TL(m \sqrt n)$. We also bound the size of the data-structure of our algorithm by $\TL(n\sqrt n)$. We also design a query algorithm with a query time $\TL(1)$. This proves the main result of the paper. 
 
 At the root of $\TT$,  except for the recursions,  we claim that constructing all other data-structures  take $O(m \sqrt{n})$ time. This is beacuse, the construction time is dominated by the time to construct $\DEP()$, which using  \Cref{lem:depconstruction}, is $O(m\sqrt n)$.    At the second level of the tree $\TT$, we have two nodes. In the left child, we have the graph $\GM \cup X$. This graph  has $m_{\GM} + n_{\GM}$ edges and $n_{\GM}$ vertices. Again applying  \Cref{lem:depconstruction}, the time taken to construct all the data-structures in the left child of root is $(m_{\GM}+n_{\GM})\sqrt n$. In the right child of the root, we have the graph $\GN \cup Y$. This graph has $m_{\GN} + n_{\GN}$ edges and $n_{\GN}+1$ vertices. The $+1$ is for the new root in $\GN$. Again applying  \Cref{lem:depconstruction}, the time taken to construct all the data-structures in the right child of root is $(m_{\GN}+n_{\GN})\sqrt n$. Thus, the total time taken at the second level of $\TT$ is    = $(m_{\GM}+n_{\GM}) \sqrt{n} + (m_{\GN}+n_{\GN}) \sqrt{n}$. Since $m_{\GM}+m_{\GN} \le m$ and $n_{\GM} + n_{\GN} = n+1$, the total time taken is  $\le (m+n+1) \sqrt n$. Note that $n_{\GM} + n_{\GN} = n+1$ because $r$ is shared both by  $\GM$\ and $\GN$.  Since, the number of nodes in $\TT$ is $O(n)$,  we claim that the number of vertices shared by sibling graphs at any level of $\TT$  is $O(n)$. Similar to the second level, we claim that the time taken at  level $\ell$ is $\TL((m +n +$ \#nodes shared at level $\ell$$)\sqrt  n) = \TL((m+n)\sqrt n)$.  We can assume that our graph $\GG$ is connected as  we need not even process a component that is not reachable from our source $s$. Thus, the previous running time bound is equal to $\TL(m \sqrt n)$. Since the height of the tree is $\TL(1)$, the total time taken to construct our data-structure is $\TL(m\sqrt n)$.
  Using the same argument, we can bound the size of the data-structure of our algorithm by $\TL(n\sqrt n)$.

  \subsection{The Query Algorithm}
  
  In this section, we will design our query algorithm that will take $s,t,e$ as its parameter. Additionally, it also takes the root of the tree $\TT$ as a parameter which contains data structures of the main graph $\GG$.  The algorithm then basically goes over all the possible cases described in   \Cref{sec:detail} (Please see Algorithm 3). Also, the algorithm compares that output with the best candidate departing path given by Algorithm 2 and returns the minimum among them.

  The reader can see that the time taken by the  algorithm (excluding recursion) is $\TL(1)$. Since, at each step in this algorithm, we either go to the left child of a node in the tree $\TT$ or to the right child, the number of recursive steps in this algorithm is $\TL(1)$. This implies that the running time of the algorithm is $\TL(1)$. Thus, we have proven the main theorem of the paper.

 
 
 

==> figures.tex <==
\section{Figures}

\input{sect51.tex}

\input{sect52.tex}

\input{lemma51.tex}

\input{LCA.tex}

\input{fig_b46.tex}







==> secsec.tex <==

\subsection{Detour point on $sc$ path and merging point on $td$ path}
\label{sctd}
We begin this section by describing the data structures utilized. Specifically, we define $\DD_{digits}^3(s,t,d_1,d_2,i,j  )$ to store the pair of edges $(e_1^*,e_2^*)$ that maximizes the distance from $s$ to $t$ subject to conditions determined by various parameters. Formally,
$$\DD_{digits}^3(s,t,n_1,n_2,i,j) = {\arg\max}_{F \in E \times E}\{ \text{conditions that depends on $s, t, d_1, d_2, i$ and $j$} \}$$


Also, we will also store the path   $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{digits}^3(s,t,n_1,n_2,i,j) $.
Here, $digits$ is set of size two with elements as $0,1$ or $2$. We maintain this as a size two array. The values of digits, $digits[0]$ and $digits[1]$ stores information about which kind of $s$ and $t$ we are dealing with. In this part, we may not always directly get a $s$ or $t$ clean vertex or intermediate vertex. We may get some vertex which act as some kind of `helper'  vertex. To denote that we use the digit $2$. We have $n_1, n_2$ depending on the distances from $s$ and $t$. Once we get $s$-clean or $t$-clean vertices through which the path $P$ passes, we can also use them in $d_1,d_2$ to ensure that the vertex we get are also $s$-clean or $t$-clean. The numbers $i,j$ is some extra condition on distance on primary path which is intact. For non-zero $i$, we assume that $2^i$ distance on the primary path from $s$ is intact. Also, $i,j$ can only be non-zero if and only if $digits[0]=2$ and $digits[1]=2$, respectively. Similary, $j$ from for $t$.So, depending on the values of $digits$.

\begin{enumerate}
        \item $digits=00$. In this case, the data-structure is  $\DD_{00}^3(s,t,d_1,d_2,i,j)$ which maximises the $st$ distance with the condition that, $d_1$ and $d_2$ distances from $s$ and $t$ respectively on both the primary and secondary path are intact from failures.
        
        \item $digits=10$. In this case, the data-structure is  $\DD_{10}^3(s,t,p,d_2,i,j)$ which maximises the $st$ distance with the condition that, the path after avoiding the faulty pair passes through $s$-clean vertex $p$ and $d_2$ distance from $t$ is intact from failures on both the primary and secondary path.
        
        \item $digits=01$. In this case, the data-structure is  $\DD_{01}^3(s,t,d_1,q,i,j)$ which maximises the $st$ distance with the condition that, the path after avoiding the faulty pair passes through $t$-clean vertex $q$ and $d_1$ distance from $s$ is intact from failures on both the primary and secondary path.
        
        \item $digits=20$. In this case, the data-structure is  $\DD_{20}^3(s,t,d_1,d_2,i,j)$. This maximiser will be dependent on the value of $i$. If $i \neq 0$, then the condition is, $2^i$ distance on the primary path and $d_1$ distance on the secondary path from $s$ is intact from failure. Also, $d_2$ distance from $t$ on both primary and secondary path is intact from failures.
        
        \item $digits=02$. In this case, the data-structure is  $\DD_{02}^3(s,t,d_1,d_2,i,j)$. This maximiser will be dependent on the value of $j$. If $j \neq 0$, then the condition is, $2^j$ distance on the primary path and $d_2$ distance on the secondary path from $t$ is intact from failure. Also, $d_1$ distance from $s$ on both primary and secondary path is intact from failures.
        
        \item $digits=12$. In this case, the data-structure is  $\DD_{12}^3(s,t,p,d_2,i,j)$. This maximiser will be dependent on the value of $j$. If $j \neq 0$, then $2^j$ distance on the primary path and $d_2$ distance on the secondary path from $t$ is intact from failure. Also,  the path after avoiding the faulty pair passes through $s$-clean vertex $p$.
        
        \item $digits=21$. In this case, the data-structure is  $\DD_{21}^3(s,t,d_1,q,i,j)$. This maximiser will be dependent on the value of $i$. If $i \neq 0$, then $2^i$ distance on the primary path and $d_1$ distance on the secondary path from $s$ is intact from failure. Also,  the path after avoiding the faulty pair passes through $t$-clean vertex $q$.
        
        \item $digits=11$. In this case, the data-structure is  $\DD_{11}^3(s,t,p,q,i,j)$with condition that, the path after avoiding the faulty pair passes through $s$-clean vertex $p$ and $t$-clean vertex $q$.
        
        \item $digits=22$.  In this case, the data-structure is  $\DD_{22}^3(s,t,d_1,d_2,i,j)$. This will be combination of 6 and 7 depending on values of $i,j$. 

        
        
\end{enumerate}




We describe our algorithm now.

Let $F=\{e_1,e_2 \}$ be the set of edges we need to avoid. Also let, $e_1=(a,b)$ and $e_2=(c,d)$. We also assume that only one fault is on the primary path. If both the faults are on the primary path then it is in the previous case \Cref{satb} . Let $e_1$ be the edge on the primary path. Now, we call the data structure $\DD_{00}^2(s,t,d_1,d_2,0,0)$ where $d_1= \min \{ |se_1|,|se_2| \}$ and $d_2=\min \{|te_1|,|te_2| \}$. Depending on what is the value of $d_1$ and $d_2$, we further divide it into cases.

\textbf{Case 1 ($d_1 =|se_2|$ and $d_2=|te_2|$) :} In this case, it is easy to observe that we either get an $s$-clean or $t$-clean vertex or intermediate vertex. Now, if the vertex we get is $s$-clean then we call $\DD_{10}^3(s,t,p,d_2,0,0)$ where $d_2=|tb|$. After that, symmetrically to the previous section, we either get a $t$-clean vertex or an intermediate vertex. 

\textbf{Case 2 ($d_1 =|se_1|$ and $d_2=|te_2|$) :} In this case, we can get either an $s$-clean or $t$-clean vertex or we can get a vertex on $sc$ path itself.  We can determine whether it is an $s$-free vertex or a vertex on $sc$ path by checking the $LCA$ of that vertex with $c$. (Or maybe by checking whatever we check in the pseudocode). Now, if we get an $s$-clean vertex then it is symmetric to the previous case (Case 1).

If the vertex, $p$ is on the shortest $sc$ path, then we can simply have $sp$ and call our data structure for $pt$ distance avoiding $F$. Now, if the primary path $pt$ contains $e_2$ then we are in \Cref{satb} and we can simply calculate the distance.

Else, we call $\DD_{20}^3(p,t,d_1,d_2,i,0)$ where $d_1 = |pe_2|, d_2=|te_2|$ and $i$ is such that, $2^i \leq |pe_1| < 2^{i+1}$. Now, similar to \Cref{sctb}, we will get an $s$-clean or $t$-clean vertex or intermediate vertex. 

Case 3 and Case 4 are symmetric to Case 2.
\newpage
 
    \begin{algorithm}
$d_1 =\min \{ |se_1|, |se_2| \} ,d_2 = |te_2|$\;
%\textbf{If} $i=0$ \textbf{then} $dist[0] = 2^{\lfloor \log |se_1|\rfloor}$ \textbf{else} $dist[0] = |se_1|$

%\textbf{If} $j=0$ \textbf{then} $dist[1] = 2^{\lfloor \log |te_2|\rfloor}$ \textbf{else} $dist[0] = |te_1|$
$digits=00$\;
$i= \lfloor \log (se_1) \rfloor$ \; 
$j= \lfloor \log ( te_2) \rfloor$ \;



 $M \leftarrow \DD_{digits}(s,t,d_1,d_2,i,j)$ \tcc*{ $M$ is edge set returned and $L$ is length of path returned }
$L \leftarrow \PP\DD_{digits}(s,t,d_1,d_2,i,j)$\;
 $\AN= L$\  \tcc*{If maximising pair does not intersects with P}

 \For{ $x \in V(M)$}
 {
    \If{$sx \cap F \neq \phi $ and $tx \cap F \neq \phi$}
    {
        $\AN= \min \{\AN, \QFT_{00}(s,x,r-1,\phi)+\QFT_{00} (x,t,r-1,\phi) \} $\;
    }
    \ElseIf{$sx \cap F = \phi$}
    {
        \If{$digits[0] =0$\ and $T_s(x)$ does not contain any faults }
        {
            $digits[0] \leftarrow 1$\;
            $clean[0] \leftarrow x$\;
            $\AN= \min \{\AN, \QFT_{digits}(s,t,r, clean) \} $\;

        }
        \ElseIf{$digits[0] =0$ and $T_s(x)$ contains any faults $(cd)$}
        {   
            $digits[0] \leftarrow 2$ \;
            

    }

            $\AN= \min \{\AN, |sx|\ +\ \QFT_{digits} (x,t,r,clean) \} $\;
        }
        \ElseIf{$digits[0] =2$ and $T_s(x)$ does not contain any fault }
        {   
            $digits[0] \leftarrow 1$ \;
            $clean[0] \leftarrow x$\;
            $\AN= \min \{\AN,  \ \QFT_{digits} (s,t,r,clean) \} $\;
        }


    }
    \ElseIf{$tx \cap F = \phi$}
    {
        \tcp{A code symmetric to the  code from line 10 to 23}
    }
    

    
   
  }

\textbf{return} \AN \;
\caption{ $\QFT_{bits} (s,t,r,clean) $:  Query algorithm for $|st \diamond F |$ where $F=\{ e_1,e_2 \}$, $r=|F|$ in case \ref{sctb}}
\label{alg:algcase2}
\end{algorithm}



\input{both.tex}

\input{deleted.tex}





==> two_n_4.tex <==

\subsection{Detour point on $sc$ path and merging point on $tb$ path}
\label{sctb}
We begin this section by describing the data structures utilized. Specifically, we define $\DD_{digits}^2(s^{i},t^{j},dist,clean)$ to store the pair of edges $(e_1^*,e_2^*)$ that maximizes the distance from $s$ to $t$ subject to conditions determined by various parameters. Formally,
\begin{equation}
\label{eq:eq3}
\DD_{digits}^2(s^i,t^j,dist,clean) = {\arg\max}_{F \in E^2}\{ \text{conditions that depends on $s, t,  i,j,dist $ and $clean$} \}
\end{equation}

Also, we will also store the path   $st \diamond \{e_1^*,e_2^*\}$ as $\PP \DD_{digits}^2(s^i,t^j,dist,clean) $.
Here, $digits$ is set of size two with elements as $0,1$ or $2$. We maintain this as a size two array. The values of digits, $digits[0]$ and $digits[1]$ stores information about which kind of $s$ and $t$ we are dealing with. In this part, we may not always directly get a $s$ or $t$ clean vertex or intermediate vertex. We may get some vertex which act as some kind of `helper'  vertex. To denote that we use the digit $2$.

\todo{Write this afterwards} For non-zero $i$, we assume that $2^i$ distance on the primary path from $s$ is intact. Also, $i,j$ can only be non-zero if and only if $digits[0]=2$ and $digits[1]=2$, respectively. Similarly, $j$ from for $t$. 

Since each cell of digits can take three values, there are 9 versions of our maximizer. We describe the conditions of the maximizer succinctly:
\begin{enumerate}
        \item $digits[0]=0$
        
        This implies that we have not found a $s$-clean vertex.
        
        Conditions in  \Cref{eq.eq3}:  $dist[0]$ distance from $s$ on both the primary and secondary path are intact from failures. If $i=0$, $dist[0]$ is a power of 2, else it is $O(2^i)$.
        
        \item $digits[0]=1$
        
        This implies that we have found a $s$-clean vertex which is stored in $clean[0]$. Let us assume that $p = clean[0]$.

Conditions in  \Cref{eq.eq3}:  The $sp$ path is intact from failures and $p$ is $s$-clean from failures. 
        
        \item $digits[0]=2$. 
        
        In this case, we have found a helper vertex such that there exists an $\EL$ such that $2^{\EL}$ distance on the primary path remains intact. Also, $dist[0]$ distance on the secondary path is intact of failures. If $i=0$, then $dist[0]$ is a power of 2, else it is $O(2^i)$.
\end{enumerate}

The conditions remain symmetric for digits[1]. The only difference is that we will calculate all distances from $t$ rather than $s$. For completeness, we define on of the maximizers. In this maximizer, we will assume that $clean[0] =p$ and $clean[1]= 2^{\EL}$.

$$
\DD_{12}(s^i,t^j,dist,clean) =
\text{argmax}_{\{e_1^*,e_2^*\} \in E^2}
\begin{cases}
 \text{ $sp$ is intact of faults $\{e_1^*,e_2^*\}$ and $p$ is $s$-clean from  $\{e_1^*,e_2^*\}$ and,  } \\
 \text{$dist[1]$ distance from $t$ on secondary path is intact from faults where}\\
\text{if $j= 0$, then $dist[1]$ is a power of 2 else it is $O(2^j)$ and}\\
\text{$2^{\EL}$ distance from $t$ on the primary path are intact of failures} 
\end{cases}
$$



Before describing our algorithm, let us state a small fact that follows from the definition of the shortest paths.
\begin{lemma}
\label{lem:switch}
Let $P = st \DIA F$. Let us assume that $e_1$ lies on the primary path $st$ and $e_2$ lies on the secondary path $st \DIA e_1$.
Let $p$ be the first vertex on $P$ from $s$ such that (1)$sp$ in intact from faults and (2) $e_2$ lies on the  shortest path $pt$. Then, for all $p' \in pe_2$, $e_1$ cannot lies on $p'
t$. 
\end{lemma}

We now describe our algorithms
Let $F=\{e_1,e_2 \}$ be the set of edges we need to avoid. Also let, $e_1=(a,b)$ and $e_2=(c,d)$. We also assume that $e_1$ is on the primary path. For our algorithm, we will maintain the following invariant:

\begin{invariant}
\label{inv:inv2}
At any point in the query algorithm, if $\QFT_{bits}(s^i,t^j,dist,clean)$ is called, then
\begin{enumerate}
\item If $i \neq 0$, then  $|sc| = O(2^i)$
\item If $j \neq 0$, then  $|tb| = O(2^j)$
\end{enumerate}
\end{invariant}

Note the difference between the above invariant and \Cref{inv:inv2}. In the previous section, the detour of path $P$ started on the primary path but here the detour starts on the secondary path. Thus, we have this difference.


 
 Like our data-structure $\DD$, $\QFT2$ also comes with nine  flavours.  We will initially call our query algorithm using the following parameters: $\QFT2_{00}(s^0,t^0,r,\phi)$. Note that the \Cref{inv:inv2} hold at this call since $i=j=0$. Since $bits = 00$,  we have not found any clean vertex till now. This can be also inferred from the fact that our fourth parameter is an empty set.   In general, we look at  four cases for $\QFT2_{digits}(s^i,t^j,dist, clean)$ depending upon the parameter $bits$. For all these cases, the following operations are common. Let $d_1 = \min\{|se_1|,|se_2|\}$ and $d_2 = |te_1|$.  If $i=0$, then we set $dist[0]$ to  the greatest power of 2 less than $d_1$. Similar is the case of $j$.
\todo{why is this difference there?}

After this, we find $\DD_{bits}(s^i,t^j,dist,clean)$. Let $\{\EO,\ET\}$ be the edges returned by the maximser. Using \Cref{lem:notinpathP}, if $\EO,\ET \notin P$, then $\PP_{bits}(s^i,t^j, dist, clean) = |P|$. For the rest of the section, let us assume that at least one edge in $\{\EO,\ET\}$ is  in the path $P$. Let us now look at the nine cases in details which we deal looking at the value of $digits[0]$ and $digits[1]$. 

\begin{enumerate}
\item $digits[0]=0$

In this case, we have not found a $s$-clean vertex. There are two cases here: 
\begin{enumerate}
\item $i=0$

If $i=0$, then we had set $dist[0] = 2^{\lfloor \log d_1\rfloor}$. In the worst case, let us assume  that $x$ is neither an intermediate or a $s$-clean vertex.  If $d_1 = |se_1|$, then we claim with a high probabily, $sx$ will contain a vertex $y$ in $\LL_{\EL_1}$ such that the distance $|ye_1| = O(2^{\EL_1})$. Now, we can call $\QFT_{digits}(y^{\EL_1},t^j,r,clean)$. We have to now show that we have made some progress. If $|yt|$ path passes through $e_1$, then in the next call, we will definitely find an intermediate, clean or a helper vertex. However, if the $yt$ path passes through $e_2$, then there is a switch in the shortest path from $st$ to $yt$. But according to \Cref{lem:switch}, this switch can happen only once. Hence, in both the cases, we make some progress. 

If $d_1 = |se_2|$, then  again we remain on $se_2$ path and the distance $|ye_2|$ is bounded by $O(2^{\EL_2})$. Also, $\min\{ye_1,ye_2\} = ye_2$.


\item $i \neq 0$

If $d_1 =|se_2|$  we either get an $s$-clean or $t$-clean vertex or intermediate vertex.\todo{why} 


If $d_1 =|se_1|$, we can get either an $s$-clean or $t$-clean vertex or we can get a vertex on $sc$ path itself.  We can determine whether it is an $s$-free vertex or a vertex on $sc$ path by checking the $LCA(x,c)$. Now, if we get an $s$-clean vertex then it is same as the above case.

The tricky case is, if the vertex in the intersection of $P$ and the maximising pair be $p$ is on the path $sc$. 
 At first, we prove two claims useful in this case.


\begin{claim}
\label{claim:trap}
        Let $P$ be the path $st \diamond \{e_1,e_2 \}$. Let $p$ be the intersecting vertex of $P$ and the maximising pair returned by $\DD_{digits}^2(s^i,t^j,dist,clean)$ where $dist[0]=|se_1|$. Let $a$ be the vertex closer to $s$ where $e_1=(a,b)$. Then, for any $x \in P[p,t]$, $|xa \diamond F| > \epsilon |P[p,x]|$.  This implies that, $a$ is not in the trapezoid of the path $P[p,t]$.
\end{claim}
\begin{proof}
        Let $|sa|=d_1$. Now, by the condition of $\DD_{digits}$, $P[s,p] \geq d_1$. 
        
        For contradiction, let $a$ be in the trapezoid of the subpath $P[p,t]$. Then, there exists a vertex $x$ on $P[p,t]$ such that $|xa| \leq \epsilon |P[p,x]|$.
        So, this will give us $|xa \diamond F |  < |px|$. Then, $|sa|+|ax \diamond F| < d_1+|px| \leq |P[s,p]|+|px|=P[s,x]$. Then, this contradicts with the fact that, $P = st \diamond \{e_1,e_2 \}$.
        So, our assumption was wrong. Hence, for any $x \in P[p,t]$, $|xa \diamond F| > \epsilon |P[p,x]|$. \end{proof}


\begin{claim}
\label{claim:LCA}
        Let $y=LCA(e_1,e_2)$. Then there is an $i \in \mathbb{N}$ such that $(1+\epsilon)^{i}<|py|<(1+\epsilon)^{i+1}<|pa|$. 
\end{claim}

\begin{proof}
        For this, let us choose the highest integer $i$ such that $(1+\epsilon)^{i}<|py|<(1+\epsilon)^{i+1}$. Now, let $|pa|<(1+\epsilon)^{i+1}$. Then, $|ya| \leq (1+\epsilon)^{(i+1)}-(1+\epsilon)^{i}=(1+\epsilon)^i(1+\epsilon-1)=\epsilon (1+\epsilon)^{i} \leq \epsilon |py|$. This violates  \Cref{claim:trap}. Hence, our assumption was wrong.
\end{proof}


Now, we further divide the cases depending on whether the primary path $xt$ contains $e_1$ or $e_2$. 

\begin{enumerate}
\item $e_1$ is the edge on primary path $pt$

Now, we set $clean[0] = (1+\EP)^i$ we get from the previous claim and $digit[0]=2$. And $p$ becomes our helper vertex. This completes our description of this case.




\item $e_2$ is the edge on primary path $pt$ 

Thus, there is a switch in the primary path from $s$ to $p$. 
By \Cref{lem:switch}, no more switches can happen on $pe_2$ path. Thus, we again call the function $\QFT(p^0,t^j,dist,clean)$.
Again, we claim that we have made some progress.

 
\end{enumerate}

\end{enumerate}
\item $digits[0] = 1$

In this case, we have already found a clean vertex, say $p$. Like \Cref{}, we claim that edge returned by the maximizer can hits $sp$ or $T_s(p)$. Thus, we may only get a clean vertex again from $s$. In the best case, we will get an intermediate vertex. 

\item $digits[1] =2$

This implies that $s$ is a helper vertex. Also, by \Cref{}, $a$ does not lie in the trapezoid of $P[s,t]$.  Let $x$ be a vertex returned by the maximizer.  We claim that either, we will go near $e_2$ or  we will get either an $s$- clean vertex or $t$-clean vertex. 
\end{enumerate}
 
\begin{algorithm}[H]
$d_1 =\min \{ |se_1|, |se_2| \} ,d_2 = |te_2|$\;
\textbf{If} $i=0$ \textbf{then} $dist[0] = 2^{\lfloor \log d_1\rfloor}$ \textbf{else} $dist[0] = d_1$\;

\textbf{If} $j=0$ \textbf{then} $dist[1] = 2^{\lfloor 
\log d_2\rfloor}$ \textbf{else} $dist[1] = d_2$\;

$\EL_1= \lfloor \log d_1 \rfloor$ \; 
$\EL_2= \lfloor \log d_2 \rfloor$ \;

\textbf{If} $digits[0]=2$ \textbf{then} $clean[0] = 2^{\EL_1}$\; 
\textbf{If} $digits[1]=2$ \textbf{then} $clean[1] = 2^{\EL_2}$\; 



 $M \leftarrow \DD_{digits}(s,t,d_1,d_2,i,j)$ \tcc*{ $M$ is edge set returned and $L$ is length of path returned }
$L \leftarrow \PP\DD_{digits}(s,t,d_1,d_2,i,j)$\;
 $\AN= L$\  \tcc*{If maximising pair does not intersects with P}

 \For{ $x \in V(M)$}
 {
    \If{$sx \cap F \neq \phi $ and $tx \cap F \neq \phi$}
    {
        $\AN= \min \{\AN, \QFT_{00}(s^0,x^0,r-1,\phi)+\QFT_{00} (x^0,t^0,r-1,\phi) \} $\;
    }
    \ElseIf{$sx \cap F = \phi$}
    {
        \If{$digits[0] \in \{0,2\}$ and $T_s(x)$ does not contain any faults }
        {
            $digits[0] \leftarrow 1$\;
            $clean[0] \leftarrow x$\;
            $\AN= \min \{\AN, \QFT_{digits}(s,t,r, clean) \} $\;

        }
        \ElseIf{$digits[0] =\{0,2\}$ and $T_s(x)$ contains any faults }
        {   
            \If{$i=0$ and $xt$ path contains $e_1$}
            {
                                Let $y$ be a vertex in $\LL_{\EL_1}$ in $sx$ path\;
                $\AN= \min \{\AN, |sy|\ +\ \QFT_{digits} (y^{\EL_1},t^j,r,clean) \} $\;                
            }
            \ElseIf{$i=0$ and $xt$ path contains $e_2$}
            {
                $\AN= \min \{\AN, |sx|\ +\ \QFT_{digits} (x^0,t^j,r,clean) \} $\;                
            }
            \Else{
            $digits[0] \leftarrow 2$\;
         
            $\AN= \min \{\AN, |sx|\ +\ \QFT_{digits} (x^0,t^j,r,clean) \} $\;
            }
        }
        
    }
    \ElseIf{$tx \cap F = \phi$}
    {
        \tcp{A code symmetric to the  code from line 10 to 23}
    }
    

    
   
  }

\textbf{return} \AN \;
\caption{ $\QFT_{bits} (s^i,t^j,r,clean) $:  Query algorithm for $|st \diamond F |$ where $F=\{ e_1,e_2 \}$, $r=|F|$ in case \ref{sctb}}
\label{alg:algcase2}
\end{algorithm}




\input{secsec.tex}
\input{both.tex}
\input{deleted.tex}




